Designing Large Foundation Models for Efficient Training and Inference: A Survey

This paper focuses on modern efficient training and inference technologies on foundation models and illustrates them from two perspectives: model and system design. Model and System Design optimize LLM training and inference from different aspects to save computational resources, making LLMs more efficient, affordable, and more accessible. The paper list repository is available at https://github.com/NoakLiu/Efficient-Foundation-Models-Survey.

==> contents/applications-new.tex <==
\section{Efficient LLM Inference in Applications}

Deploying LLMs in practical applications requires balancing computational efficiency, latency, and accuracy. Optimizations such as model compression, memory management, and retrieval-augmented generation (RAG) are implemented to ensure scalable and responsive systems. This section explores specific application domains, emphasizing deployment-specific challenges and solutions.

\subsection{Real-Time Virtual Assistants}

Virtual assistants, such as customer service bots or personal assistants (e.g., Siri, Alexa), must deliver low-latency responses while managing computational resources effectively. One common strategy is early-exit mechanisms that terminate computations once confidence in the response surpasses a deployment-defined threshold:
\begin{align}
    \mathcal{C}^{(l)} = g(W^{(l)}, X^{(l)}),
\end{align}
where $\mathcal{C}^{(l)}$ represents the system's confidence metric at layer $l$, $W^{(l)}$ are the model parameters, and $X^{(l)}$ are the activations. 

Deployment systems define an early-exit condition:
\begin{align}
    \mathcal{C}^{(l)} > \tau, \quad \hat{y} = \text{argmax}(\mathcal{C}^{(l)}),
\end{align}
where $\tau$ is a threshold chosen based on latency-accuracy trade-offs. 

This approach ensures virtual assistants deliver responses within milliseconds. For example, systems discussed in \citep{Li_Wang_Chen_2024} achieve a 30\% latency reduction with minimal accuracy loss.

\subsection{Batch Processing in Search Engines}

Search engines process high query volumes, making batch processing essential for optimizing throughput. Queries $\{q_1, q_2, \dots, q_B\}$ are grouped into batches to maximize hardware utilization. For a batch of $B$ queries:
\begin{align}
    \mathcal{Y} = f(\mathcal{Q}; W),
\end{align}
where $\mathcal{Q} = \{q_1, q_2, \dots, q_B\}$ are query embeddings, $W$ are model parameters, and $\mathcal{Y}$ are the results. 

Batch latency is minimized by leveraging parallel hardware:
\begin{align}
    T_{\text{batch}} = \frac{C_{\text{total}}}{P},
\end{align}
where $C_{\text{total}}$ is the total computational cost, and $P$ is the number of processing units.

For example, batching methods similar to \citep{wei2024feature, yang2024advancing} improve throughput in e-commerce search engines, handling millions of queries per second with low latency.

\subsection{Domain-Specific Retrieval-Augmented Generation (RAG)}

RAG integrates external data sources to enhance LLM performance in knowledge-intensive domains such as finance and healthcare. For a query $q$, RAG retrieves relevant documents $\{d_1, \dots, d_k\}$ from an external database:
\begin{align}
    \mathcal{R} = \text{Retrieve}(q, \mathcal{D}),
\end{align}
where $\mathcal{D}$ is the document database and $\mathcal{R}$ contains the top-$k$ retrieved documents.

The retrieved documents are concatenated with the query and passed to the LLM for inference:
\begin{align}
    \mathcal{Y} = \text{LLM}(q, \mathcal{R}),
\end{align}
where $\mathcal{Y}$ is the generated response.

Systems like \citep{lewis2020retrieval} reduce hallucinations and improve factual accuracy, enabling reliable deployment in critical applications.

\subsection{Streaming Inference in Cybersecurity}

Cybersecurity applications demand real-time threat detection over continuous data streams. To minimize latency, streaming inference divides data into windows $\{x_1, x_2, \dots, x_T\}$ and processes each window independently:
\begin{align}
    y_t = f(x_t; W_t),
\end{align}
where $x_t$ is the input at time $t$, $W_t$ represents the model parameters, and $y_t$ is the predicted output.

Real-time deployment systems overlap computation and communication:
\begin{align}
    T_{\text{stream}} = \max(T_{\text{compute}}, T_{\text{transfer}}),
\end{align}
ensuring that threat detection operates continuously with minimal delays.

Recent advancements like \citep{zhou2023efficientstreaming} demonstrate the scalability of these methods for high-throughput environments, enabling real-time protection against cyber threats.

\subsection{Latency-Accuracy Trade-Offs in Edge Deployments}

Edge deployments in IoT and autonomous systems demand lightweight models with stringent latency requirements. A typical deployment pipeline involves compressing models to reduce their memory footprint:
\begin{align}
    W_{\text{compressed}} = \text{Compress}(W, \alpha),
\end{align}
where $\alpha$ controls the compression ratio. The compressed weights are optimized for edge hardware with limited resources:
\begin{align}
    \mathcal{L} = \|f(X; W_{\text{compressed}}) - f(X; W)\|^2 + \lambda \cdot C_{\text{memory}},
\end{align}
where $\mathcal{L}$ is the loss function balancing accuracy and memory cost.

Techniques discussed in \citep{han2023iotcompression} achieve up to 50\% reduction in memory usage while maintaining competitive accuracy for real-time IoT deployments.


==> contents/applications.tex <==
% \section{Application}

% Some applications such as \cite{yang2024advancing} using compressed models for emotional analysis, while applications such as \cite{Li_Wang_Chen_2024}, \cite{wei2024feature}, \cite{JIPD7671} deploying compressed models in large-scale financial circumstances. Model compression of LLMs also widely used in cybersecurity aspects such as \cite{weng2024leveraging}, \cite{Weng2024}, \cite{Weng202404}, and \cite{Weng202406}.

\section{Efficient LLM Inference in Applications}

Deploying LLMs in practical applications requires balancing computational efficiency, latency, and accuracy. Optimizations such as model compression, memory management, and RAG are applied across industries to ensure LLMs perform effectively in real-time systems, finance, cybersecurity, and healthcare. Below, we examine how efficient inference techniques improve performance in specific application domains, each supported by relevant references.

\subsection{Real-Time Virtual Assistants}
Virtual assistants, like those in customer service or personal assistants (e.g., Siri, Alexa), must provide fast and accurate responses. Implementing early-exit strategies allows the model to halt computations once a sufficient confidence level is reached, optimizing response times. This ensures users receive fast and accurate results without noticeable delays.

Applications like those discussed in \citep{Li_Wang_Chen_2024} demonstrate the effectiveness of such strategies in high-traffic customer service scenarios, reducing response time and improving user experience.

\subsection{Batch Processing in Search Engines}
Search engines and recommendation systems process vast numbers of queries simultaneously. By grouping multiple queries into batches, these systems optimize throughput while maintaining low latency. Batch processing is critical in high-demand environments such as e-commerce platforms, where quick and relevant search results enhance user experience and increase sales.

Batch processing techniques similar to those used in \citep{wei2024feature, yang2024advancing} allow search engines and recommendation systems to handle thousands of queries per second, improving overall performance in large-scale operations.

\subsection{RAG for Knowledge-Intensive Tasks}
In tasks that require accurate and up-to-date information, such as technical support, legal research, and open-domain question answering, Retrieval-Augmented Generation (RAG) integrates external knowledge retrieval into the generation process. This enables LLMs to provide responses that are both contextually relevant and grounded in the latest information.

Systems like \textit{REALM} \citep{guu2020realm} and \textit{RAG} \citep{lewis2020retrieval} demonstrate how RAG enhances LLM performance in customer service and research assistance by retrieving external documents and integrating them into generated responses.


==> contents/mm_system.tex <==
\subsection{System Design for Multi-Modality LLMs}

Efficient key-value (KV) caching is essential for accelerating inference in multi-modal LLM systems, particularly when integrating diverse modalities like text, image, and audio. By leveraging the unique characteristics of each modality and their interdependencies, advanced KV cache designs can optimize both memory usage and computational efficiency. This section explores multi-modal KV caching strategies, focusing on unified representations, compression techniques, and sophisticated eviction mechanisms.

\subsubsection{Unified Multi-Modal KV Cache Representations}

\paragraph{Multi-Modal Key and Value Structures}

Unified KV representations reduce redundancy while capturing cross-modal dependencies. For a multi-modal input \( x = \{x_t, x_i, x_a\} \) (text, image, and audio, respectively), the KV cache can be structured as:

\[
K = \begin{bmatrix}
W_k^{(t)} h^{(t)} & \alpha_{ti} W_k^{(i)} h^{(i)} & \alpha_{ta} W_k^{(a)} h^{(a)} \\
\alpha_{it} W_k^{(t)} h^{(t)} & W_k^{(i)} h^{(i)} & \alpha_{ia} W_k^{(a)} h^{(a)} \\
\alpha_{at} W_k^{(t)} h^{(t)} & \alpha_{ai} W_k^{(i)} h^{(i)} & W_k^{(a)} h^{(a)}
\end{bmatrix},
\]

where \( W_k^{(m)} \) and \( h^{(m)} \) represent the projection matrix and hidden state for modality \( m \). The coefficients \( \alpha_{mn} \) denote learned alignment weights between modalities \( m \) and \( n \), enabling efficient cross-modal interaction \citep{MS-ALIGN, MS-Flamingo, MS-M3AE}.

\paragraph{Joint Cross-Modal Attention-Based Compression}

Given the computational overhead of storing full KV caches, cross-modal attention matrices \( A \) can be used to guide compression. For text \( T \) and image \( I \), the attention matrix is:

\[
A_{TI} = \text{diag}(K_T^\top Q_I) + \text{diag}(K_I^\top Q_T),
\]

where \( Q \) and \( K \) represent the query and key matrices, respectively. A low-rank approximation of \( A_{TI} \) via Singular Value Decomposition (SVD) yields:

\[
A_{TI} \approx U_{TI} \Sigma_{TI} V_{TI}^\top, \quad \Sigma_{TI} = \text{diag}(\sigma_1, \sigma_2, \dots, \sigma_r),
\]

where \( U_{TI}, \Sigma_{TI}, V_{TI} \) are the top-\( r \) components. This reduced-rank representation balances efficiency and accuracy \citep{MS-PerceiverIO, MS-LowRankFusion}.

\subsubsection{Advanced Cache Eviction Policies Leveraging Multi-Modality}

\paragraph{Cross-Modal Sensitivity-Based Eviction}

Cache eviction in multi-modal systems must account for both intra-modal and cross-modal contributions. The sensitivity of the model output \( y \) to a key \( k_t^m \) from modality \( m \) is defined as:

\[
S_t^{(m)} = \left\| \frac{\partial y}{\partial k_t^m} \right\|_2^2 + \sum_{n \neq m} \beta_{mn} \left\| \frac{\partial y}{\partial k_t^n} \cdot \frac{\partial k_t^n}{\partial k_t^m} \right\|_2^2,
\]

where \( \beta_{mn} \) captures the dependency strength between modalities \( m \) and \( n \). Entries with the smallest \( S_t^{(m)} \) are evicted, ensuring minimal performance degradation \citep{MS-SensitivityCache, MS-MultimodalHessian}.

\paragraph{Hessian-Aware Cross-Modal Eviction}

Second-order optimization methods are useful for assessing the importance of cache entries. The Hessian-aware importance of a key \( k_t^m \) is computed as:

\[
\Delta \mathcal{L} = \frac{1}{2} \left( \frac{\partial \mathcal{L}}{\partial k_t^m}^\top H_t^{(m)} \frac{\partial \mathcal{L}}{\partial k_t^m} + \sum_{n \neq m} \frac{\partial \mathcal{L}}{\partial k_t^m}^\top H_t^{(mn)} \frac{\partial \mathcal{L}}{\partial k_t^n} \right),
\]

where \( H_t^{(m)} \) is the Hessian for modality \( m \), and \( H_t^{(mn)} \) captures cross-modal dependencies. Cache entries with minimal \( \Delta \mathcal{L} \) are prioritized for eviction, preserving critical cross-modal interactions \citep{MS-Flamingo, MS-HessianEviction}.

\paragraph{Entropy-Regularized Cross-Modal Eviction}

Maintaining diversity in cache content can be achieved through entropy-based eviction. The joint entropy of a key distribution \( p_t^{(m,n)} \) across modalities \( m \) and \( n \) is:

\[
H_t = - \sum_{m \in \mathcal{M}} \sum_{n \in \mathcal{M}} p_t^{(m,n)} \log p_t^{(m,n)},
\]

where \( p_t^{(m,n)} \) is the normalized attention contribution of \( k_t \) for modalities \( m \) and \( n \). Entries with low \( H_t \) are evicted, promoting diversity and informativeness \citep{MS-EntropyCache, MS-MultimodalFusion}.


==> contents/others.tex <==
% \section{Other Optimizations for LLM Inference}

% \subsection{Memory Scheduling and Efficient Inference}
% \subsubsection{Memory Scheduling for Large Model Inference}
% Efficient memory scheduling is crucial for managing LLMs' massive memory footprint during inference. Techniques like \textit{FlashAttention} \cite{dao2022flashattention} reduce the overhead of memory access by using chunked computation, minimizing storage requirements for intermediate results. This technique is especially important for long-sequence tasks, where memory usage can quickly become a bottleneck.

% \subsubsection{Context Compression with Sentinel Tokens}
% \textit{Context Compression} with sentinel tokens \cite{wang2023context} introduces an approach that compresses redundant context information in long-sequence tasks, reducing the memory burden and improving computational efficiency during inference. This technique is particularly useful for applications like dialogue systems that require long-context processing.

% \subsubsection{Heavy-Hitter Oracle for Efficient Inference}
% \textit{H2O} \cite{zhang2023h2o} presents an oracle-based framework for efficient generative inference by focusing computational resources on ``heavy-hitter'' tokens—those with high probability of occurrence. By prioritizing these tokens, H2O reduces overall inference time, ensuring better efficiency for systems like GPT and PaLM.

% \input{tables/LLMs}

% \subsection{Distributed Training and Parallelism}
% \subsubsection{Distributed Training for Large Models}
% Distributed training techniques, such as model and data parallelism, are essential for managing LLM inference at scale. Systems like \textit{Megatron-LM} \cite{shoeybi2019megatron} and \textit{Colossal-AI} \cite{xu2021colossal} partition the model and data across multiple GPUs, achieving efficient training and inference for models with billions of parameters.

% \subsection{Fine-Tuning and Compression}
% \subsubsection{Fine-Tuning with Parameter Efficiency}
% Full model fine-tuning is often impractical for large LLMs due to resource constraints. Parameter-efficient techniques like \textit{Low-Rank Adaptation (LoRA)} \cite{hu2021lora} enable fine-tuning of a small subset of parameters, adapting models like GPT-3 and PaLM for specific tasks without extensive retraining.

% \subsubsection{Sentinel Tokens and Context Compression}
% The \textit{Context Compression} method using sentinel tokens \cite{wang2023context} compresses long context sequences, reducing memory requirements and preserving important information for accurate token generation in tasks like summarization and dialogue.

% \section{Other Optimizations for LLM Inference}

% Optimizing LLM inference requires a multifaceted approach, addressing challenges related to memory management, computational efficiency, and scalability. Techniques such as memory scheduling, context compression, and token prioritization, along with distributed training and fine-tuning, play critical roles in improving the performance of large models. Below, we explore these optimizations with accompanying formulas.

% \subsection{Memory Scheduling and Efficient Inference}
% \subsubsection{Memory Scheduling for Large Model Inference}
% Memory scheduling is crucial for managing the high memory demands of LLMs during inference. One approach is \textit{FlashAttention} \citep{dao2022flashattention}, which reduces memory access overhead by using chunked computation, minimizing the storage required for intermediate attention results. This approach is particularly beneficial for long-sequence tasks, where memory usage can become a bottleneck. The core mechanism of FlashAttention is:

% \begin{align}
%     \hat{A}_t = \text{softmax}\left(\frac{Q_t K_{1:t}^\top}{\sqrt{d_k}}\right) V_{1:t},
% \end{align}

% where the computation is divided into chunks, allowing for efficient memory access and reduced storage of intermediate values $\hat{A}_t$.

% \subsubsection{Context Compression with Sentinel Tokens}
% Context compression with sentinel tokens \citep{wang2023context} is another method to reduce the memory footprint in long-context tasks such as dialogue systems and document summarization. By compressing redundant context information, the system reduces the memory load while preserving critical information. The context compression process can be expressed as:

% \begin{align}
%     C_{\text{compressed}} = f\left(C_{\text{original}}, S\right),
% \end{align}

% where $C_{\text{compressed}}$ represents the compressed context, $C_{\text{original}}$ is the original long context, and $S$ denotes the sentinel tokens that help preserve important information during compression.

% \subsubsection{Heavy-Hitter Oracle for Efficient Inference}
% The \textit{H2O} framework \citep{zhang2023h2o} introduces an oracle-based approach to optimize LLM inference by focusing computational resources on high-probability, "heavy-hitter" tokens. This method ensures that only tokens with a high likelihood are prioritized, reducing overall computation. The key idea can be formalized as:

% \begin{align}
%     P(\hat{T}_t) = \argmax_{T_t} P(T_t | T_{1:t-1}),
% \end{align}

% where $P(\hat{T}_t)$ is the highest-probability token predicted at time step $t$, focusing computation only on this token to improve inference efficiency.

% \subsection{Distributed Training and Parallelism}
% \subsubsection{Distributed Training for Large Models}
% Distributed training is essential for scaling LLMs across multiple devices. Techniques such as model and data parallelism distribute the model parameters and data across GPUs, allowing efficient training and inference. Systems like \textit{Megatron-LM} \citep{shoeybi2019megatron} and \textit{Colossal-AI} \citep{xu2021colossal} apply these techniques, allowing for large-scale models to be efficiently trained and used in inference. The parallelism can be expressed as:

% \begin{align}
%     X_{\text{output}} = f_{\text{parallel}}\left(X_{\text{input}}\right),
% \end{align}

% where $f_{\text{parallel}}$ represents the distributed computation across multiple GPUs, ensuring that large-scale models can handle massive datasets and complex tasks during inference.

% \subsection{Fine-Tuning and Compression}
% \subsubsection{Fine-Tuning with Parameter Efficiency}
% Fine-tuning large models is often impractical due to the high resource requirements. Techniques like \textit{Low-Rank Adaptation (LoRA)} \citep{hu2021lora} enable parameter-efficient fine-tuning by updating only a small subset of parameters. This allows models like GPT-3 and PaLM to be adapted for specific tasks without requiring extensive retraining. The low-rank adaptation can be modeled as:

% \begin{align}
%     W_{\text{adapted}} = W + \Delta W,
% \end{align}

% where $W$ represents the original weights of the model, and $\Delta W$ is a low-rank update that adapts the model to new tasks without retraining all the parameters.

% \subsubsection{Sentinel Tokens and Context Compression}
% In addition to memory scheduling, \textit{context compression} using sentinel tokens \citep{wang2023context} allows LLMs to handle long sequences by compressing context information, reducing memory requirements while maintaining important details for inference. The compression is performed as:

% \begin{align}
%     C_{\text{compressed}} = f(C_{\text{original}}, S),
% \end{align}

% where $C_{\text{compressed}}$ is the compressed context, $C_{\text{original}}$ is the original sequence, and $S$ represents sentinel tokens that guide the compression process, helping preserve the most relevant information for inference tasks such as summarization and dialogue.

\section{Other Optimizations for LLM Inference}

Optimizing LLM inference involves multiple strategies that address memory efficiency, computational speed, scalability, and accuracy. These techniques are designed to enhance the practicality of deploying large models in resource-constrained environments while maintaining high performance. Below, we explore various optimizations, such as memory scheduling, contextual compression, distributed training, and inference accuracy.

\subsection{Memory Scheduling and Efficient Inference}
Efficient memory scheduling is crucial for managing the memory footprint of large models, especially during long-sequence tasks. Techniques like chunked computation minimize memory usage by reducing intermediate storage and optimizing memory access patterns, allowing for faster processing and scalability. 

The general memory scheduling mechanism can be written as:

\begin{align}
    M_{\text{used}} = \sum_{i=1}^{n_{\text{chunks}}} f_{\text{chunk}}\left(X_i\right),
\end{align}

where $M_{\text{used}}$ represents the total memory used during inference, $n_{\text{chunks}}$ is the number of chunks, and $f_{\text{chunk}}$ refers to the memory-efficient operation applied to each chunk $X_i$. Techniques like \textit{FlashAttention} \citep{dao2022flashattention} follow this principle by reducing memory access and intermediate storage requirements during attention calculations.

\subsection{Context Compression with Sentinel Tokens}
Context compression is another critical optimization for long-sequence tasks like dialogue and summarization. By using sentinel tokens to reduce redundant context, systems can preserve important information while decreasing memory usage. 

The operation of context compression can be described as:

\begin{align}
    C_{\text{compressed}} = \text{compress}\left(C_{\text{original}}, S\right),
\end{align}

where $C_{\text{compressed}}$ is the compressed context, $C_{\text{original}}$ is the original input context, and $S$ represents sentinel tokens that guide the compression process. This technique, employed in \textit{Context Compression} \citep{wang2023context}, improves computational efficiency without sacrificing model performance on long-context tasks.

\subsection{Heavy-Hitter Oracle for Efficient Inference}
Token prioritization techniques like the \textit{Heavy-Hitter Oracle (H2O)} \citep{zhang2023h2o} focus computational resources on high-probability tokens, improving efficiency by skipping unlikely candidates. This technique ensures that inference focuses on the most probable tokens, speeding up the overall process.

The general form for token prioritization can be expressed as:

\begin{align}
    P(T_t) = \argmax_{T_t} P(T_t | T_{1:t-1}),
\end{align}

where $P(T_t)$ is the probability of token $T_t$ at time step $t$, conditioned on the previous tokens $T_{1:t-1}$. Focusing on high-probability tokens reduces computational overhead by limiting the scope of inference to the most likely candidates.

\subsection{Distributed Training and Parallelism}
Distributed training and parallelism are essential for handling large-scale models that exceed the memory limits of a single device. By distributing model parameters and data across multiple GPUs, systems like \textit{Megatron-LM} \citep{shoeybi2019megatron} and \textit{Colossal-AI} \citep{xu2021colossal} allow for efficient scaling and training of models with billions of parameters.

A general formula for distributed parallelism can be written as:

\begin{align}
    X_{\text{output}} = f_{\text{parallel}}\left(X_{\text{input}}, W_{\text{partitioned}}\right),
\end{align}

where $f_{\text{parallel}}$ represents the function applied across different GPUs, $W_{\text{partitioned}}$ denotes the partitioned model weights across multiple devices, and $X_{\text{input}}$ is the input data. This approach maximizes hardware utilization and enables scalable training and inference.

\subsection{Retrieval-Augmented Generation (RAG) Inference}
RAG (Retrieval-Augmented Generation) integrates external knowledge retrieval with the language model's generation process, improving performance in tasks that require up-to-date or specialized knowledge. In RAG, the model retrieves relevant documents or context from a knowledge base before generating responses, which enhances both the accuracy and relevance of generated content.

The process of RAG inference can be formalized as:

\begin{align}
    X_{\text{retrieval}} = \text{Retrieve}(Q), \quad X_{\text{gen}} = f_{\text{generate}}\left(X_{\text{retrieval}}, Q\right),
\end{align}

where $Q$ is the input query, $X_{\text{retrieval}}$ represents the retrieved information from the knowledge base, and $f_{\text{generate}}$ is the generation function that incorporates the retrieved information to produce the final output $X_{\text{gen}}$. Systems like \textit{REALM} \citep{guu2020realm} and \textit{RAG} \citep{lewis2020retrieval} use this approach to enhance the performance of models on open-domain question-answering and other knowledge-intensive tasks.

\subsection{Inference Accuracy Optimization}
In addition to speed and efficiency, maintaining inference accuracy is critical for many LLM applications. Techniques like calibration and temperature scaling are used to adjust the output probabilities of LLMs to ensure that the model’s confidence aligns with its accuracy.

A general formula for temperature scaling during inference can be written as:

\begin{align}
    P(T_t | T_{1:t-1}) = \frac{\exp{\left(\frac{z_t}{T}\right)}}{\sum_{t'} \exp{\left(\frac{z_{t'}}{T}\right)}},
\end{align}

where $z_t$ represents the logits (pre-softmax values) for token $T_t$ and $T$ is the temperature parameter. Lower temperatures sharpen the probability distribution, making the model more confident in its predictions, while higher temperatures smooth the distribution. This approach helps control the trade-off between diversity and accuracy in generated outputs.

\subsection{Multi-Task Inference and Task Specialization}
As LLMs are increasingly used across diverse domains, multi-task learning becomes essential for improving inference efficiency. Multi-task inference allows models to perform various tasks (e.g., translation, summarization, QA) simultaneously, reducing the need to train separate models for each task. Task specialization further optimizes performance by fine-tuning certain portions of the model to excel in specific tasks.

The general form of multi-task inference can be expressed as:

\begin{align}
    X_{\text{task}} = f_{\text{task-specific}}\left(X_{\text{input}}, W_{\text{shared}}\right),
\end{align}

where $f_{\text{task-specific}}$ represents the task-specific function applied to the input data $X_{\text{input}}$, and $W_{\text{shared}}$ denotes the shared parameters of the model across multiple tasks. Systems like \textit{T5} \citep{raffel2020exploring} and \textit{MT-DNN} \citep{liu2019multi} employ multi-task learning to enable models to handle a wide range of tasks efficiently.

\input{tables/LLMs}

==> contents/quant_dong_cite.tex <==
\subsection{Quantization}

\subsubsection{Bit-width Based Quantization}
\subsubsubsection{2.1.1 8-bit Quantization (INT8, FP8, W8A8)}
\begin{itemize}
    \item Efficient 8-bit quantization for Transformers \cite{frantar2022optimal}.
    \item F8Net: Fixed-point 8-bit only multiplication for network quantization \cite{dettmers2023spqr}.
    \item SmoothQuant: INT8/FP8 hybrid quantization \cite{xiao2023smoothquant}.
    \item LLM.int8(): INT8 quantization optimized for Hugging Face \cite{liu2023qllm}.
    \item AKVQ-VL: Attention-aware KV cache adaptive 2-bit quantization \cite{yuan2023rptq}.
    \item Efficient Post-Training Quantization with FP8 Formats \cite{wu2023zeroquant}.
    \item Mixed Precision Training with FP8 \cite{li2023llm}.
    \item Hybrid 8-bit Floating Point (HFP8) Training \cite{sheng2023flexgen}.
\end{itemize}

\subsubsubsection{2.1.2 4-bit Quantization (W4A8, W4A4, NF4, FP4)}
\begin{itemize}
    \item QRazor: 4-bit LLM quantization with significant data razoring \cite{lee2025qrazor}.
    \item LLM-FP4: Floating-point 4-bit quantization for Transformers \cite{liu2023llmfp4}.
    \item BiDM: Extreme binarization of Diffusion Models (1-bit) \cite{zheng2024bidmpushinglimitquantization}.
    \item Q-Diffusion: Quantization-aware training for Diffusion Models \cite{li2023qdiffusion}.
    \item Atom: Low-bit quantization for efficient LLM serving \cite{zhao2023atom}.
    \item A Leap Forward in LLMs Post-Training W4A8 Quantization Using Floating-Point Formats \cite{wu2023zeroquantfp}.
    \item GPTQ: Accurate 4-bit PTQ for Transformers \cite{frantar2022gptq}.
    \item AWQ: Activation-aware quantization for LLMs and DiT-based diffusion models \cite{huang2024billm}.
    \item QuaRot: Outlier-free 4-bit inference in rotated LLMs \cite{ashkboos2024quarot}.
    \item OmniQuant: Omnidirectionally calibrated quantization \cite{shao2023omniquant}.
    \item MPQ-DM: Mixed Precision Quantization for Diffusion Models \cite{wu2023zeroquant}.
    \item ZeroQuant-FP: A leap forward in W4A8 quantization \cite{wu2023zeroquant}.
\end{itemize}

\subsubsubsection{2.1.3 2-bit \& 1-bit Quantization}
\begin{itemize}
    \item Binary Diffusion: Experimental binarization for generative models \cite{kinakh2025binary}.
    \item RotateKV: 2-bit KV cache quantization with outlier-aware rotations \cite{su2025rotatekv}.
    \item AKVQ-VL: 2-bit adaptive quantization for vision-language models \cite{su2025akvqvl}.
    \item Integer or Floating Point? New Outlooks for Low-Bit Quantization on Large Language Models \cite{tseng2024quip}.
    \item QuEST: Low-bit Diffusion Model Quantization via Efficient Selective Finetuning \cite{liu2024spinquant}.
    \item LUT-GEMM: Lookup table-based quantized matrix multiplication for efficient LLMs \cite{park2022lut}.
\end{itemize}

\input{tables/quant_machine}
\input{tables/quant_bit}

\subsubsection{Method-Based Quantization}
\subsubsubsection{2.2.1 Post-Training Quantization (PTQ)}
\begin{itemize}
    \item GPTQ: Efficient 4-bit PTQ for Transformers and Diffusion Models \cite{frantar2023gptq}.
    \item AWQ: Activation-aware quantization for LLMs and DiT-based diffusion models \cite{lin2024awq}.
    \item INT8 PTQ (ONNX, TensorRT): Optimized for high-performance inference \cite{migacz2017int8}.
    \item SmoothQuant: INT8/FP8 hybrid post-training quantization \cite{xiao2022smoothquant}.
    \item Distribution-Aware Diffusion Model Quantization via Distortion Minimization \cite{li2023distribution}.
    \item PTQD: Accurate Post-Training Quantization for Diffusion Models \cite{wu2023zeroquant}.
    \item RPTQ: Reorder-based post-training quantization \cite{yuan2023rptq}.
\end{itemize}

\subsubsubsection{2.2.2 Quantization-Aware Training (QAT)}
\begin{itemize}
    \item DoReFa-Net: Low-bit training with learned quantization functions \cite{zhou2016dorefa}.
    \item Q-Diffusion: QAT for stable diffusion acceleration \cite{li2023qdiffusion}.
    \item Ultra-Low Precision 4-bit Training for Deep Neural Networks \cite{sun2020ultra}.
    \item Memory-Efficient Optimizers with 4-bit States \cite{chen2023memory}.
    \item EfficientDM: Efficient Quantization-Aware Fine-Tuning of Low-Bit Diffusion Models \cite{yang2023efficientdm}.
\end{itemize}

\subsubsubsection{2.2.3 Mixed-Precision \& Adaptive Quantization}
\begin{itemize}
    \item AKVQ-VL: Attention-aware adaptive quantization for KV cache \cite{su2025akvqvl}.
    \item RotateKV: Adaptive rotation-based KV cache compression \cite{su2025rotatekv}.
    \item Quant-LLM: FP6-centric GPU-optimized quantization \cite{yao2023quantllm}.
    \item F8Net: Mixed-precision fixed-point quantization \cite{yang2023f8net}.
    \item MPQ-DM: Mixed Precision Quantization for Extremely Low Bit Diffusion Models \cite{yang2023mpqdm}.
    \item DilateQuant: Accurate and Efficient Diffusion Quantization via Weight Dilation \cite{zhang2023dilatequant}.
    \item Q-DM: An Efficient Low-bit Quantized Diffusion Model \cite{wu2023zeroquant}.
    \item SpinQuant: LLM quantization with learned rotations \cite{liu2024spinquant}.
\end{itemize}

==> contents/quantization.tex <==
\subsection{Quantization}
Quantization is one popular way for model compression. It selectively reduces the precision of model parameters in its 2-digit representation, thereby reducing the model's storage needs. \citep{liu2024llmeasyquanteasyuse} To simplify, quantization acts as a merchant, where the merchandise is model parameters. Large language models have billions of parameters, leading to immense storage requirements and slow inference speed. The "quantization" merchant will buy the valuable weights at a normal price (original precision) and the less important ones at a lower price (lower precision). By using this strategy, the merchant gains a small yet efficient model with less computational resources, which can be comparable in performance to the original model.

% One famous quantization method is AWQ, developed by \citet{lin2024}. In this work, the authors proposed an activation-aware quantization method. They found that the generation stage (output generation) is much slower than context (input context analysis) in on-device applications of LLMs. Further studies showed that the generation stage is bounded by memory, and memory usage can be greatly reduced by using activation compression. \citet{lin2024} also noted that skipping a small fraction of important weights (salient weights) while quantizing others (non-salient weights) can greatly reduce quantization loss. They found that selecting salient weights based on activation magnitude can improve quantization performance. The core technique of AWQ is to calculate a parameter called the channel scaling factor for the tradeoff between salient and non-salient channels. This makes the quantization process "activation aware" because the parameter is learnable, and it is computationally friendly as AWQ does not require regression or backpropagation during the quantization phase, thus needing fewer data and computational resources.

% Another popular quantization method is the integer-arithmetic-only inference developed by \citet{jacob2018}. Instead of using a low-digit floating point number for storage, they developed a new quantization scheme that only uses integers for computation during the inference stage, greatly reducing computational resources. Jacob also developed integer-only-arithmetic multiplication methods to achieve fast inference. Empirical results show that integer-only-arithmetic inference with 8-bit quantization is comparable to floating-point inference on different hardware, proving the effectiveness of integer-only quantization. 

\subsubsection{Post-Training Quantization}
Post-Training Quantization (PTQ) is a popular method that reduces model size and computational cost without requiring retraining. It is applied after a model has already been trained, thus optimizing for speed and storage efficiency while minimally impacting performance. This technique is often easier to implement than training-integrated quantization approaches, making it suitable for rapid deployment of LLMs with reduced resources.
% Post-Training Quantization is a popular method that reduces model size and computational cost without requiring retraining. It is applied after a model has already been trained, thus optimizing for speed and storage efficiency while minimally impacting performance. This technique is often easier to implement than training-integrated quantization approaches, making it suitable for rapidly deploying large language models (LLMs) with reduced resources.


\paragraph{Weight-Only Quantization} Quantizing only the model’s weights reduces memory usage and computational cost by compressing parameters. This method is straightforward but may slightly impact accuracy since activations are kept in full precision. However, applying weight-only quantization to LLMs presents challenges, especially with outliers and broad weight distribution ranges. GPTQ \cite{frantar2022gptq}, inspired by Optimal Bit Quantization (OBQ) \cite{frantar2022optimal}, addresses these challenges by structuring weight quantization in a row-wise sequence. By updating only specific portions of the Hessian matrix during quantization, GPTQ minimizes the computational overhead compared to OBQ, where frequent updates would otherwise increase complexity. Another advancement, LUT-GEMM \cite{park2022lut}, improves inference speed by employing a Look-Up Table (LUT) to accelerate dequantization, combining binary-coding quantization (BCQ) with optimized intervals to reduce computational load during inference.

Additionally, managing outliers is essential in weight-only quantization. Outliers in weight distributions can skew quantization, reducing efficiency and potentially degrading model performance. Techniques like SpQR \cite{dettmers2023spqr} and OliVe \cite{guo2023olive} address this by assigning higher precision to outliers. SpQR, for example, separates high-magnitude weights into a sparse matrix while quantizing the remaining weights to 3 bits, maintaining performance with minimal additional storage requirements. BiLLM \cite{huang2024billm} takes this further by binarizing non-salient weights and retaining higher precision only for weights deemed significant by the Hessian matrix. This approach achieves a very low-bit representation (1.08 bits on average) while keeping accuracy degradation to a minimum.

Rotation-based techniques further support weight-only quantization by reshaping weight distributions to reduce outliers. QuIP\# \cite{tseng2024quip} and QuaRot \cite{ashkboos2024quarot} apply rotation matrices to weight matrices, aligning distributions closer to Gaussian forms and enabling efficient low-bit quantization. In QuIP\#, for instance, the rotation process is achieved by the transformation $R$ and can be defined as:
\begin{equation}
\begin{aligned}
W' = R \cdot W
,
\end{aligned}
\end{equation}
where $W'$ is the original weight matrix,  $R$ is the rotation matrix, and $W$ is the rotated weight matrix. This rotation minimizes the impact of outliers, making it possible to compress weights effectively without compromising model stability. Such transformations enable extreme compression ratios, which are ideal for memory-constrained environments where activations remain in full precision.



\paragraph{Weight-Activation Quantization} Building upon Weight-Only Quantization, weight-activation quantization compresses both weights and activations, achieving substantial reductions in memory usage and computational demands. Compared to weight-only quantization, this approach requires managing the dynamic range variability of activations, which can be highly sensitive to layer-specific dependencies in LLMs. Techniques like ZeroQuant-V2 \cite{yao2023zeroquant} and LLM-MQ \cite{li2023llm} address this challenge by implementing adaptive precision allocation that adjusts according to each layer’s sensitivity to quantization. ZeroQuant-V2, for instance, introduces the Low-Rank Compensation (LoRC) technique, which uses low-rank matrices to mitigate quantization errors, effectively preserving model fidelity even at lower bit widths. ZeroQuant-FP \cite{wu2023zeroquant} further extends this by employing floating-point formats (FP8 for activations and FP4 for weights), allowing for efficient use of hardware such as NVIDIA H100 GPUs. This floating-point approach achieves significant memory savings while maintaining computational efficiency, as it leverages hardware support for FP formats.

SpinQuant \cite{liu2024spinquant} and SmoothQuant \cite{xiao2023smoothquant} employ unique methods to handle outliers in both weights and activations, facilitating more uniform quantization across layers. Specifically, SpinQuant uses learned rotation matrices (e.g., $R_1$ and $R_2$) to transform distributions offline, reshaping both weights and activations to reduce outliers. In contrast, SmoothQuant introduces a scaling factor that shifts the activation range closer to that of weights, easing the quantization process by balancing their respective distributions.

Further accuracy enhancements are achieved through error correction and adaptive adjustments across layers. QLLM \cite{liu2023qllm} and OmniQuant \cite{shao2023omniquant} employ layer-wise optimization techniques that apply gradient-based corrections to quantization errors, often using low-rank matrices. Meanwhile, Atom \cite{zhao2024atom} is designed to achieve high throughput, incorporating low-bit quantization not only for weights and activations but also for the KV cache, resulting in up to a 7.7x improvement in serving speed. These adaptive quantization methods achieve substantial memory and computational efficiency, supporting resource-intensive applications without sacrificing model accuracy.




\paragraph{KV Cache Quantization} KV cache quantization is proposed for managing memory in transformer-based LLMs, where the self-attention mechanism’s key-value (KV) pairs contribute to substantial memory costs, particularly in long-context tasks. By quantizing the KV cache, these methods make it feasible to use LLMs with extended context windows under limited memory.

Atom \cite{zhao2024atom} addresses this by applying low-bit quantization, specifically a 4-bit quantization scheme for KV pairs, which optimizes both memory and computational efficiency during self-attention. Atom employs asymmetric quantization at the attention head level, leveraging the fact that the softmax normalization in attention is less sensitive to quantization errors. FlexGen \cite{sheng2023flexgen} further enhances KV cache quantization with a three-tiered memory system, distributing data across GPU, CPU, and disk to support efficient deployment on single-GPU setups.

Rotation-based techniques, such as QuaRot \cite{ashkboos2024quarot}, improve KV cache quantization by employing randomized Hadamard rotations to achieve uniform distribution of values, allowing for end-to-end 4-bit quantization with minimal calibration overhead. Cluster-based approaches add further control by organizing activation channels with similar distributions into clusters. RPTQ \cite{yuan2023rptq} implements reorder-based clustering for KV cache quantization, where channels within each cluster are quantized independently to preserve essential attention dynamics. This precise clustering and quantization framework supports extended context-dependent tasks, such as dialogue systems and summarization, where efficient memory management is crucial. Together, these advanced techniques offer a robust and memory-efficient approach for deploying LLMs in settings that demand extensive context handling.

\subsubsection{Quantization-Aware Training (QAT)}

Quantization-Aware Training is a proactive quantization method where quantization is simulated during model training. This approach enables the model to learn with quantization noise in mind, making it more resilient to precision losses when deployed with lower bit-width formats. QAT generally achieves higher accuracy than PTQ in highly sensitive applications but comes with additional training overhead.

\paragraph{Full Model Quantization} Quantizing all model components uniformly during training enables greater efficiency but demands high computational resources. This approach maximizes compression but may require calibration to manage precision-sensitive layers. 

LLM-QAT \cite{liu2023llm} presents a data-free distillation method for LLM quantization-aware training, which allows for model quantization independent of training data, resembling post-training quantization but with added flexibility. Quantizing weights, activations, and the KV cache enables throughput improvements and handles long sequence dependencies in LLaMA models (7B, 13B, 30B) down to 4-bit precision. Large performance gains are observed in low-bit settings over training-free methods. OneBit \cite{xu2024onebit} explores an extreme 1-bit quantization for LLMs. With a unique 1-bit parameter representation and matrix decomposition-based parameter initialization, OneBit achieves at least 81\% of non-quantized model performance on LLaMA models, even under such low bit-width. The PEQA \cite{du2024bitdistiller} approach combines parameter-efficient fine-tuning (PEFT) with quantization, tuning only quantization scales to allow seamless task transitions and memory-efficient adaptation for low-bit quantized LLMs. This method achieves sub-4-bit precision while retaining language modeling and few-shot learning performance comparable to full-precision LLMs. LoftQ \cite{li2023loftq}, a LoRA-fine-tuning-aware quantization framework, tackles performance degradation in quantized LLMs. By jointly quantizing the model and initializing low-rank adapters for LoRA fine-tuning, it enhances downstream task generalization, particularly in the challenging 2-bit and 2/4-bit mixed precision ranges. L4Q \cite{jeon2024l4q} merges quantization-aware training (QAT) with LoRA, optimizing memory overhead and achieving superior performance in sub-4-bit settings. By employing a memory-efficient layer design, L4Q successfully balances full model quantization and fine-tuning effectiveness, making it a robust QAT solution for resource-intensive language tasks. EfficientQAT \cite{chen2024efficientqat} introduces a two-stage quantization-aware training approach to address memory limitations in LLMs. The method consists of block-wise training of all parameters (Block-AP), followed by end-to-end quantization parameter training (E2E-QP), which allows for reduced accuracy loss in low-bit settings. EfficientQAT proves effective across a range of models and quantization bits, such as achieving 2-bit quantization on LLaMA-2-70B with minimal accuracy degradation. EdgeQAT \cite{shen2024edgeqat} addresses inference speed and computational efficiency for deploying LLMs on edge devices by quantizing weights, activations, and KV cache with entropy-guided quantization and token importance-aware adaptation. By dynamically adjusting quantization for tokens, EdgeQAT demonstrates substantial acceleration (up to 2.37x) compared to FP16 models on edge devices while maintaining task accuracy.

\paragraph{Partial Quantization} Selectively quantizing specific layers (e.g., attention layers) balances efficiency with performance by keeping critical areas in higher precision. Partial Quantization suits applications where some layers are more sensitive to precision loss than others.
 
BitDistiller \cite{du2024bitdistiller} integrates quantization-aware training (QAT) with knowledge distillation (KD) to reach ultra-low precisions (sub-4-bit). Through asymmetric quantization, clipping, and a Confidence-Aware Kullback-Leibler Divergence (CAKLD) objective, BitDistiller achieves fast convergence and high performance in 3-bit and 2-bit configurations, requiring fewer training resources. QLoRA \cite{dettmers2023qlora} leverages a 4-bit NormalFloat (NF4) data type, double quantization, and paged optimizers for efficient memory management, enabling 65B parameter models to be fine-tuned on a single 48GB GPU. The approach provides scalability in resource-limited environments while retaining model performance across diverse benchmarks and model scales. QA-LoRA \cite{xu2023qa} combines quantization-aware training with low-rank adaptation to enable efficient tuning and deployment of quantized models. It employs group-wise operators, enhancing quantization flexibility while managing adaptation overhead. QA-LoRA achieves high accuracy with reduced memory and time requirements on the LLaMA models. IR-QLoRA \cite{qin2024accurate} is a novel approach that enhances quantization accuracy through information retention mechanisms, including Information Calibration Quantization for accurate parameter retention and Information Elastic Connection for LoRA fine-tuning. IR-QLoRA shows significant accuracy improvements on LLaMA models in 2-4 bit settings with minimal additional time costs. 

==> contents/quantization_p.tex <==
\subsection{Quantization}

Quantization is a popular method for model compression that selectively reduces the precision of model parameters, thereby decreasing storage requirements and computational costs. To simplify, quantization can be likened to a merchant trading model parameters: valuable weights are retained at full precision, while less important ones are represented at reduced precision. This strategy results in a smaller, more efficient model with minimal performance degradation. Large language models, with billions of parameters, benefit greatly from quantization as it addresses their immense storage needs and slow inference speeds \citep{lin2024, jacob2018}.

\subsubsection{Post-Training Quantization (PTQ)}

Post-Training Quantization (PTQ) is widely adopted to reduce model size and computational cost without retraining. PTQ operates on pre-trained models, making it efficient for deployment with minimal performance impact. It is particularly advantageous for rapid deployment of large language models (LLMs) in resource-constrained environments \citep{frantar2022gptq, park2022lut}.

\paragraph{Weight-Only Quantization}
Weight-only quantization compresses model parameters, reducing memory usage and computational requirements. However, challenges such as handling outliers and broad weight distribution ranges must be addressed. Techniques like GPTQ \citep{frantar2022gptq} and LUT-GEMM \citep{park2022lut} optimize weight quantization, with GPTQ using row-wise quantization and LUT-GEMM employing look-up tables for faster dequantization. Advanced methods like SpQR \citep{dettmers2023spqr} and OliVe \citep{guo2023olive} tackle outliers by assigning higher precision to significant weights. Further, rotation-based approaches, such as QuIP\# \citep{tseng2024quip} and QuaRot \citep{ashkboos2024quarot}  employ rotation matrices to align weight distributions, enabling effective compression while preserving model stability.

\paragraph{Weight-Activation Quantization}
Weight-activation quantization extends weight-only quantization by compressing both weights and activations. Techniques like ZeroQuant-V2 \citep{yao2023zeroquant}, SmoothQuant \citep{xiao2023smoothquant}, and SpinQuant \citep{liu2024spinquant} address activation outliers and dynamic range variability. ZeroQuant-V2 employs Low-Rank Compensation (LoRC) to mitigate errors, while SmoothQuant scales activations to balance distributions. These methods enhance efficiency, achieving significant memory savings without compromising performance.

\paragraph{KV Cache Quantization}
KV cache quantization addresses the memory overhead caused by storing key-value pairs in transformer-based LLMs. Atom \citep{zhao2024atom} applies low-bit quantization to KV pairs, optimizing memory and computational efficiency. FlexGen \citep{sheng2023flexgen} uses a three-tiered memory system for efficient deployment on single-GPU setups. Rotation-based techniques, such as QuaRot \citep{ashkboos2024quarot}, further enhance KV cache quantization by uniformizing value distributions, enabling efficient compression even in long-context tasks.

\subsubsection{Quantization-Aware Training (QAT)}

Quantization-Aware Training (QAT)~\citep{tao2022compression} introduces quantization noise during model training, enabling models to adapt to reduced precision formats. Compared to PTQ, QAT typically achieves better performance in low-bit settings but requires additional training resources.

\paragraph{Full Model Quantization}
Full model quantization applies uniform precision across all model components. Techniques like LLM-QAT \citep{liu2023llm} and BitDistiller \citep{du2024bitdistiller} optimize for extreme compression by leveraging distillation and gradient-based corrections. LoRA-based methods, such as LoftQ \citep{li2023loftq} and L4Q \citep{jeon2024l4q}, enhance downstream task performance by jointly optimizing quantization and low-rank adaptation.

\paragraph{Partial Quantization}
Partial quantization selectively applies low precision to certain layers while retaining others at full precision. QLoRA \citep{dettmers2023qlora} and QA-LoRA \citep{xu2023qa} implement selective quantization strategies with group-wise operators, enabling scalability and adaptability in resource-limited environments. Techniques like IR-QLoRA \citep{qin2024accurate} enhance accuracy by retaining critical information during quantization.

\subsubsection{Conclusion}
Quantization offers a spectrum of methods for compressing large language models, from post-training approaches like GPTQ \citep{frantar2022gptq} to advanced quantization-aware training frameworks such as EdgeQAT \citep{shen2024edgeqat}. These methods enable the deployment of efficient, low-resource LLMs without significant performance loss, making quantization a cornerstone of modern model compression strategies.


==> contents/text_system.tex <==
\section{System Design for Text LLM}

% make a table to conclude all the formula involved
\input{contents/KVcache}

\subsection{KV Cache Design}

Key-Value (KV) caching is an essential technique in Transformer-based large language models (LLMs), significantly reducing the computational overhead associated with autoregressive sequence generation. By precomputing and reusing key ($\mathbf{K}$) and value ($\mathbf{V}$) matrices, KV caching enables efficient handling of self-attention across long contexts.

\subsubsection{Mathematical Framework of KV Caching}

In the self-attention mechanism \citep{vaswani2017attention}, the attention computation for a sequence of $t$ tokens is given by:
\begin{equation}
    \mathbf{A}_t = \text{softmax}\left(\frac{\mathbf{Q}_t \mathbf{K}_{1:t}^\top}{\sqrt{d_k}} + \mathbf{B}_t\right),
\end{equation}
where $\mathbf{A}_t \in \mathbb{R}^{n_t \times n_t}$ represents the attention weights, $\mathbf{Q}_t, \mathbf{K}_{1:t}, \mathbf{V}_{1:t}$ are the query, key, and value matrices, $d_k$ is the key dimension, and $\mathbf{B}_t$ introduces relative positional biases \citep{raffel2020exploring}. The output representation $\hat{\mathbf{X}}_t$ is then computed as:
\begin{equation}
    \hat{\mathbf{X}}_t = \mathbf{A}_t \mathbf{V}_{1:t}.
\end{equation}

To avoid redundant computations, KV caching incrementally stores key-value matrices:
\begin{equation}
    \text{Cache Update:} \quad \mathbf{K}_{1:t+1} = \left[\mathbf{K}_{1:t}; \mathbf{K}_{t+1}\right], \quad \mathbf{V}_{1:t+1} = \left[\mathbf{V}_{1:t}; \mathbf{V}_{t+1}\right].
\end{equation}

\subsubsection{Advanced KV Cache Formulations}

\begin{itemize}
    \item   \textbf{Low-Rank Approximation} \citep{huang2023cachegen, xiong2024uncomp}:
To reduce memory consumption, the key and value matrices are represented in a compressed, low-rank form:
\begin{equation}
    \tilde{\mathbf{K}} = \mathbf{U} \mathbf{K}, \quad \tilde{\mathbf{V}} = \mathbf{V} \mathbf{V},
\end{equation}
where $\mathbf{U}, \mathbf{V} \in \mathbb{R}^{r \times d_k}$ are learned projection matrices, and $r \ll d_k$ is the reduced rank. The resulting attention computation is:
\begin{equation}
    \mathbf{A}_t = \text{softmax}\left(\frac{\mathbf{Q}_t \mathbf{U} \mathbf{K}_{1:t}^\top}{\sqrt{r}}\right).
\end{equation}

\item \textbf{Query-Aware Sparsity} \citep{chen2023quest, wan2024look, wan2024d2o, liu2024graphsnapshotgraphmachinelearning}:
KV caching can be further optimized by updating only the most relevant entries dynamically. The sparsity mask $\mathbf{M}_t$ is defined as:
\begin{equation}
    \mathbf{M}_t = \text{top-}k\left(\left|\frac{\mathbf{Q}_t \mathbf{K}_{1:t}^\top}{\sqrt{d_k}}\right|\right),
\end{equation}
where $\text{top-}k(\cdot)$ selects the indices of the top-$k$ attention scores. Sparse keys and values are then expressed as:
\begin{equation}
    \mathbf{K}_{\text{sparse}} = \mathbf{M}_t \odot \mathbf{K}_{1:t}, \quad \mathbf{V}_{\text{sparse}} = \mathbf{M}_t \odot \mathbf{V}_{1:t},
\end{equation}
where $\odot$ denotes element-wise multiplication.
\end{itemize}

\subsubsection{Optimizations Across Inference Stages}

During the prefilling stage, key-value matrices are computed for all tokens in the input sequence:
\begin{equation}
    \mathbf{K}_t = f_K(\mathbf{X}_t; \theta), \quad \mathbf{V}_t = f_V(\mathbf{X}_t; \theta),
\end{equation}
where $f_K$ and $f_V$ are learnable transformations. Techniques such as rotary embeddings \citep{su2021roformer} enhance efficiency:
\begin{equation}
    \mathbf{K}_t = \cos(\omega t) \mathbf{K}_t + \sin(\omega t) \mathbf{K}_t^\perp,
\end{equation}
where $\omega$ is the rotational frequency, and $\mathbf{K}_t^\perp$ represents the orthogonal component.

During decoding, cached matrices are reused, with attention computation for step $t'$ formulated as:
\begin{equation}
    \hat{\mathbf{X}}_{t'} = \text{softmax}\left(\frac{\mathbf{Q}_{t'} \mathbf{K}_{1:t'}^\top}{\sqrt{d_k}}\right) \mathbf{V}_{1:t'}.
\end{equation}

% \subsubsection{Impact of KV Cache Optimizations}

% 1. \textbf{Latency Reduction}:
% Compression (\textit{CacheGen}) and sparse updates (\textit{Quest}) reduce time-to-first-token (TTFT) and accelerate decoding.

% 2. \textbf{Memory Efficiency}:
% PagedAttention \citep{zhao2023vllm} manages memory across GPU and CPU, leveraging virtual mapping:
% \begin{equation}
%     \text{Paged Cache:} \quad \text{KV}_{\text{virtual}} = \text{Translate}(\text{KV}_{\text{GPU}}, \text{KV}_{\text{CPU}}).
% \end{equation}

% 3. \textbf{Scalability}:
% Low-rank and sparse representations enable efficient inference for long-context sequences without significant memory growth.

\subsubsection{Impact of KV Cache Optimizations}

\begin{itemize}
    \item \textbf{Latency Reduction}:  
    Techniques such as compression (\textit{CacheGen}) and sparse updates (\textit{Quest}) significantly reduce time-to-first-token (TTFT) and expedite the decoding process.
    
    \item \textbf{Memory Efficiency}:  
    PagedAttention \citep{zhao2023vllm} improves memory management by dynamically leveraging virtual mapping across GPU and CPU. This mechanism can be expressed as:  
    \[
    \text{Paged Cache:} \quad \text{KV}_{\text{virtual}} = \text{Translate}(\text{KV}_{\text{GPU}}, \text{KV}_{\text{CPU}}).
    \]
    
    \item \textbf{Scalability}:  
    By employing low-rank and sparse representations, these optimizations enable efficient inference for long-context sequences while maintaining minimal memory growth.
\end{itemize}


\subsection{Token Reduction}
Token reduction methods aim to decrease the number of tokens processed by transformer models, reducing computational complexity while maintaining the model's performance. These methods are effective in both large language models (LLMs), visual LLMs such as Vision Transformers (ViTs), or Mamba~\citep{shen2024famba}. Below, we discuss several token reduction techniques, including token pruning and token merging, along with their mathematical formulations.

\subsubsection{Token Pruning}
Token pruning seeks to eliminate redundant or less important tokens during inference or training. This method dynamically reduces the token set based on pre-defined criteria or learned importance scores. Token pruning in LLMs and visual transformers must ensure that the critical information from pruned tokens is retained by the remaining tokens to minimize performance degradation.

Let $T \in \mathbb{R}^{n \times d}$ represent the token matrix, where $n$ is the number of tokens and $d$ is the token dimension. The pruning mask $M \in \{0, 1\}^n$ determines which tokens to retain, where $M_i = 0$ indicates that token $i$ is pruned. The objective function can be expressed as:

\begin{align}
    \argmin_M \|T \odot M - \tilde{T}\|_2^2,
\end{align}

where $\tilde{T}$ represents the remaining token matrix after pruning. The pruning decision often relies on token importance scores derived from attention mechanisms or heuristics like magnitude-based pruning \citep{rao2021dynamicvit, yin2022avit}.

\paragraph{Attention-based Pruning:} In methods like DynamicViT \citep{rao2021dynamicvit}, attention scores $A \in \mathbb{R}^{n \times n}$ are used to rank tokens by their relevance. The tokens with the lowest cumulative attention scores across layers are pruned. The cumulative importance score for each token $i$ can be defined as:

\begin{align}
    S_i = \sum_{l=1}^L \sum_{j=1}^n A_{ij}^{(l)},
\end{align}

where $L$ denotes the number of transformer layers.

\paragraph{Magnitude-based Pruning:} In magnitude-based pruning \citep{goyal2020powerbert}, tokens are pruned based on their $\ell_2$ norm in the feature space. The smallest magnitude tokens are removed:

\begin{align}
    S_i = \|T_i\|_2,
\end{align}
where $T_i$ is the $i$-th token vector.

\subsubsection{Token Merging}
Token merging, unlike pruning, combines similar tokens to reduce the token count while preserving information. Token Merging (ToMe) \citep{bolya2023tome} is an effective method for both LLMs and ViTs, which merges tokens based on their similarity in feature space. This technique maintains a consistent number of tokens across inputs, facilitating batched inference.

Let $T \in \mathbb{R}^{n \times d}$ represent the token matrix, where each row is a token. Token merging combines similar tokens $(i, j)$ to form a merged token $\hat{T}_k$:

\begin{align}
    \hat{T}_k = \alpha T_i + (1 - \alpha) T_j,
\end{align}
where $\alpha \in [0,1]$ is a weighting factor based on token similarity. Cosine similarity is often used to measure the similarity between tokens:

\begin{align}
    \text{sim}(T_i, T_j) = \frac{T_i^\top T_j}{\|T_i\| \|T_j\|}.
\end{align}

\paragraph{Proportional Attention:} To prevent merged tokens from losing their influence in self-attention, proportional attention \citep{bolya2023tome} adjusts the attention mechanism by accounting for the size of each merged token. The modified attention matrix $A$ is given by:

\begin{align}
    A = \text{softmax}\left(\frac{QK^\top}{\sqrt{d}} + \log(s)\right),
\end{align}
where $s$ is a vector representing the number of tokens each merged token represents.

\subsection{Optimization Techniques for Efficient LLMs}

Optimizing large language models (LLMs) involves reducing memory and computational costs while maintaining performance. This section outlines dynamic cache allocation, sparsity-aware computation, precision scaling, and parallelism strategies with mathematical formulations and references to state-of-the-art methods.

\subsubsection{Dynamic KV Cache Allocation}

Efficient memory allocation dynamically adjusts the KV cache size based on token importance \citep{vlcache, pyramidkv}:
\begin{align}
    C_{\text{KV}}^{(l)} = \sum_{i=1}^{N_t} M_{i,l} \cdot \text{Size}_{\text{token}},
\end{align}
where $M_{i,l} \in \{0, 1\}$ indicates whether token $i$ is retained at layer $l$.

Compressed KV cache optimizes memory further \citep{smoothquant}:
\begin{align}
    \text{KV}_{\text{compressed}}^{(l)} = \sum_{t=1}^{N_t} \left[M_{t,l} \cdot \text{Quant}(X_t, b_t)\right],
\end{align}
where $\text{Quant}(X_t, b_t)$ applies $b_t$-bit quantization, dynamically adjusted per token.

\subsubsection{Sparsity-Aware Computation}

Sparsity in attention reduces redundant calculations \citep{quest, shen2023flexgen}:
\begin{align}
    A_{\text{sparse}}^{(l)} = M^{(l)} \odot \text{softmax}\left(\frac{Q^{(l)} K^{(l) \top}}{\sqrt{d_k}}\right),
\end{align}
where $M^{(l)}$ is a binary mask selecting relevant tokens.

Query-aware sparsity retains the top-$k$ tokens with the highest attention scores \citep{quest, pyramiddrop}:
\begin{align}
    M_{i,j}^{(l)} = 
    \begin{cases} 
    1, & \text{if } \text{Rank}(a_{i,j}^{(l)}) \leq k, \\
    0, & \text{otherwise}.
    \end{cases}
\end{align}

\subsubsection{Precision Scaling}

Dynamic precision adjusts computations to balance cost and accuracy \citep{micikevicius2018mixed, smoothquant}:
\begin{align}
    C_{\text{compute}}^{(l)} = \sum_{i=1}^{N_p} \alpha_{i,l} \cdot C_{\text{FP32}} + (1 - \alpha_{i,l}) \cdot C_{\text{FP16}},
\end{align}
where $\alpha_{i,l}$ indicates the proportion of FP32 precision operations.

Low-bit quantization reduces memory usage \citep{llmint8}:
\begin{align}
    W_q = \text{round}\left(\frac{W}{\Delta}\right) \cdot \Delta, \quad \Delta = \frac{W_{\max} - W_{\min}}{2^b - 1}.
\end{align}

\subsubsection{Distributed and Asynchronous Execution}

\textbf{Parallelism:} Model and pipeline parallelism distribute computations across GPUs \citep{megatronlm, shen2023flexgen}:
\begin{align}
    X_{\text{output}}^{(l)} = \sum_{i=1}^N f_{\text{GPU}_i}^{(l)}(X_{\text{input}}^{(l)}).
\end{align}

Pipeline parallelism overlaps computations \citep{flexgen, megatronlm}:
\begin{align}
    T_{\text{pipeline}} = \frac{\sum_{l=1}^L C_{\text{forward}}^{(l)}}{1 + \text{Overlap}},
\end{align}
where $\text{Overlap}$ measures concurrent execution efficiency.

\textbf{Asynchronous Decoding:} Token generation and attention are parallelized \citep{flashdecoding++}:
\begin{align}
    \hat{X}_t = \text{softmax}\left(\frac{Q_t K_{1:t}^\top}{\sqrt{d_k}}\right) V_{1:t} + \Delta_t,
\end{align}
where $\Delta_t$ captures corrective updates.

\subsubsection{General Optimization Objective}

The overall optimization combines compute, cache, and precision costs \citep{vlcache, quest, micikevicius2018mixed}:
\begin{align}
    \min_{M, P, Q} \sum_{l=1}^L \left(\|X_{\text{true}} - X_{\text{pred}}\|^2 + \lambda_1 C_{\text{compute}}^{(l)} + \lambda_2 C_{\text{KV}}^{(l)} + \lambda_3 C_{\text{precision}}^{(l)}\right),
\end{align}
where $M$ is the sparsity mask, $P$ defines parallelism configurations, $Q$ specifies precision levels, and $\lambda_1, \lambda_2, \lambda_3$ are trade-off parameters.

==> contents/tllm-sys.tex <==
\subsection{System Design for Text LLMs}

%
% \input{figures/KVcache_sys}


Text Large Language Models (LLMs) face significant challenges in managing computational and memory costs during autoregressive generation. Effective system design leverages optimizations like Key-Value (KV) caching, token reduction, and precision scaling to balance efficiency and accuracy. These methods are grounded in mathematical frameworks that formalize the trade-offs between model performance and resource utilization.

\subsubsection{KV Cache Design}

\input{figures/KVcacheop}

Key-Value (KV) caching is a cornerstone of transformer-based LLMs, significantly reducing computational overhead by reusing previously computed key (\(\mathbf{K}\)) and value (\(\mathbf{V}\)) matrices. During autoregressive generation, the self-attention mechanism computes the output for a sequence of tokens by leveraging the precomputed cache. Let \(\mathbf{Q}_t\), \(\mathbf{K}_{1:t}\), and \(\mathbf{V}_{1:t}\) denote the query, key, and value matrices at time \(t\). The attention mechanism scales the query-key interaction by the inverse square root of the key dimension \(d_k\), applies positional biases \(\mathbf{B}_t\), and generates the final representation \(\hat{\mathbf{X}}_t = \text{softmax}((\mathbf{Q}_t \mathbf{K}_{1:t}^\top)/\sqrt{d_k} + \mathbf{B}_t) \mathbf{V}_{1:t}\). To improve memory efficiency, advanced KV cache compression methods use low-rank approximations, where keys and values are projected into lower-dimensional spaces using learned projection matrices \(\mathbf{U}\) and \(\mathbf{V}\). Specifically, the compressed representations are given by \(\mathbf{K}_{\text{low}} = \mathbf{U} \mathbf{K}\) and \(\mathbf{V}_{\text{low}} = \mathbf{V} \mathbf{V}^\top\), where \(r \ll d_k\) controls the rank of the approximation. Query-aware sparsity further optimizes KV caching by dynamically identifying and updating only the most relevant tokens using a sparsity mask \(\mathbf{M}_t\), defined as the top-\(k\) entries of the scaled query-key scores. This hierarchical approach combines memory reduction and computational efficiency while maintaining the fidelity of attention outputs.

The general optimization for KV cache design balances memory usage, computational cost, and attention fidelity, expressed as:
\[
\min_{\mathbf{K}_{\text{low}}, \mathbf{V}_{\text{low}}} \| \mathbf{K} - \mathbf{K}_{\text{low}} \|_F^2 + \| \mathbf{V} - \mathbf{V}_{\text{low}} \|_F^2 + \lambda \cdot \mathcal{C}(\mathbf{K}_{\text{low}}, \mathbf{V}_{\text{low}}),
\]
where \(\mathcal{C}(\mathbf{K}_{\text{low}}, \mathbf{V}_{\text{low}})\) models the memory and computational costs of the compressed representations \citep{huang2023cachegen, xiong2024uncomp}.

\subsubsection{Token Reduction Strategies}

Token reduction focuses on minimizing the number of tokens processed during training and inference while retaining essential information for accurate predictions. In transformer models, tokens often exhibit redundancy, particularly in the deeper layers where contextualized embeddings converge. Let \(T \in \mathbb{R}^{n \times d}\) denote the token embeddings, where \(n\) is the token count and \(d\) is the embedding dimension. Token pruning techniques dynamically identify and remove less important tokens based on learned importance scores or predefined heuristics. Importance scores can be computed using attention weights, token magnitudes, or cumulative relevance across layers. For example, attention-based pruning ranks tokens by their cumulative importance \(S_i = \sum_{l=1}^L \sum_{j=1}^n A_{ij}^{(l)}\), where \(A^{(l)}\) represents the attention matrix at layer \(l\). Tokens with the lowest scores are removed, and their information is redistributed to the remaining tokens. Alternatively, token merging methods combine similar tokens, reducing the total count while preserving overall representation. In methods like Token Merging (ToMe), merged tokens are computed as weighted combinations, where similarity scores guide the merging process. The merged embeddings \(\hat{T}_k = \alpha T_i + (1 - \alpha) T_j\), with \(\alpha\) determined by cosine similarity, ensure that merged tokens retain meaningful features. These approaches effectively reduce computational costs in both text and visual transformer architectures.

The optimization objective for token reduction can be formulated as:
\[
\min_{M, \hat{T}} \|T \odot M - \hat{T}\|_F^2 + \mu \cdot \text{Cost}(M) + \nu \cdot \text{Regularization}(M),
\]
where \(M \in \{0, 1\}^n\) is the token retention mask, \(\text{Cost}(M)\) captures the computational overhead, and \(\text{Regularization}(M)\) enforces structural constraints \citep{bolya2023tome, rao2021dynamicvit}.

\subsubsection{Unified Optimization Framework}

Combining KV cache design and token reduction strategies requires a unified framework to balance trade-offs between computational cost, memory usage, and model accuracy. Let \(\mathcal{L}_{\text{task}}(X, \theta)\) denote the primary task loss, where \(X\) is the input data and \(\theta\) represents model parameters. The unified optimization framework jointly considers token selection, KV compression, and sparsity:
\[
\min_{M, \mathbf{K}_{\text{low}}, \mathbf{V}_{\text{low}}} \mathcal{L}_{\text{task}}(X, \theta) + \lambda_1 \|T \odot M - \hat{T}\|_F^2 + \lambda_2 \| \mathbf{K} - \mathbf{K}_{\text{low}} \|_F^2 + \lambda_3 \mathcal{C}(\mathbf{K}_{\text{low}}, \mathbf{V}_{\text{low}}),
\]
where \(\lambda_1, \lambda_2, \lambda_3\) are hyperparameters balancing the contributions of token reduction, KV compression, and computational cost. This framework integrates pruning, merging, and precision scaling techniques to optimize LLM performance across diverse tasks \citep{huang2023cachegen, bolya2023tome, rao2021dynamicvit}.


==> contents/tllm.tex <==
% \subsection{Architecture Optimization and Parallelism}
\subsection{Architecture Optimization and Parallelism}
Architecture optimization and parallelism are essential techniques for enhancing the efficiency of LLMs by reducing computational complexity, leveraging hardware resources effectively, and minimizing inference latency. These optimizations include asynchronous execution, model and pipeline parallelism, mixed precision inference, and contextual sparsity. A general mechanism to improve inference efficiency can be expressed by distributing computations across devices and selectively skipping unnecessary operations:

\begin{align}
    \hat{X}_t = f_{\text{parallel}}\left(Q_t, K_{1:t}, V_{1:t}\right) \cdot M_t,
\end{align}

where $f_{\text{parallel}}$ represents the parallelized computation of attention and MLP operations across multiple devices, $K_{1:t}$ and $V_{1:t}$ are the cached key and value matrices, and $M_t$ is a sparsity mask applied to skip irrelevant computations, optimizing both memory and computational resources.

% \subsubsection{Contextual Sparsity in MLP and Attention Blocks}
% A critical optimization for LLM inference is leveraging contextual sparsity in Multi-Layer Perceptrons (MLPs) and attention mechanisms. Activation functions such as ReLU or GeLU induce sparsity, creating opportunities to skip zero-value computations without compromising accuracy \cite{kurtz2020inducing}. Systems like \textit{FlexGen} \cite{shen2023flexgen} and \textit{Deja Vu} \cite{li2022deja} utilize sparsity prediction mechanisms to reduce computation during inference. The \textit{Quest} system \cite{chen2023quest} extends this by introducing query-aware sparsity mechanisms, focusing on long-context inference and skipping irrelevant token computations.

\subsubsection{Contextual Sparsity in MLP and Attention Blocks}
Contextual sparsity is a key optimization technique for LLM inference, particularly in the Multi-Layer Perceptrons (MLPs) and attention blocks of transformers. Activation functions like ReLU and GeLU induce sparsity by producing zero values for certain inputs, which creates opportunities to skip unnecessary computations without compromising accuracy \citep{kurtz2020inducing}. The sparsity of activations can be expressed as:

\begin{align}
    X_{\text{sparse}} = f(X) \quad \text{where} \quad f(x) = \text{ReLU}(x) = \max(0, x),
\end{align}

where $X_{\text{sparse}}$ represents the sparse activations generated by the ReLU function. Systems like \textit{FlexGen} \citep{shen2023flexgen} and \textit{Deja Vu} \citep{li2022deja} leverage sparsity prediction mechanisms to skip these zero-value computations during inference, thereby reducing the overall computational cost.

In addition to activation sparsity, \textit{Quest} \citep{chen2023quest} introduces query-aware sparsity, which selectively skips irrelevant token computations based on the query context. The mechanism predicts token relevance for long-context inference by applying a sparsity mask:

\begin{align}
    M_t = \text{top-k}\left(\left|\frac{Q_t K_t^\top}{\sqrt{d_k}}\right|\right),
\end{align}

where $M_t$ is the sparsity mask that selects the top-$k$ most relevant tokens based on their attention scores. This optimization reduces the number of token computations, especially in scenarios with long input sequences, making the inference process more efficient.


% \subsubsection{Asynchronous Execution for Parallelism}
% \textit{FlashDecoding++} \cite{wang2023flashdecoding} introduces asynchronous execution techniques for LLM inference, allowing predictions to be computed concurrently with token generation. This reduces latency and ensures smoother inference by decoupling prediction tasks from the main inference process.

% \subsubsection{Model Parallelism and Pipeline Execution}
% Model parallelism is a key technique for scaling LLMs across multiple devices. Frameworks like \textit{Megatron-LM} \cite{shoeybi2019megatron} and \textit{FlexGen} \cite{shen2023flexgen} use model parallelism to distribute the model across GPUs, ensuring efficient utilization of hardware resources. Similarly, pipeline parallelism distributes different layers of the model across devices, reducing sequential processing bottlenecks.

% \subsubsection{Mixed Precision and Low-Bit Inference}
% Mixed precision training is widely used to reduce memory and computation costs, where non-critical operations are executed in FP16 or BF16 precision \cite{micikevicius2018mixed}. Extending this, \textit{Fast and Efficient 2-bit LLM Inference} \cite{zhou2023efficient} presents a low-bit inference approach that uses 2/4/16-bit weight matrices, combined with asynchronous dequantization to maintain accuracy while reducing memory bandwidth.

\subsubsection{Asynchronous Execution for Parallelism}
Asynchronous execution enables concurrent computations during LLM inference, significantly reducing latency by overlapping token generation with prediction calculations. In \textit{FlashDecoding++} \citep{wang2023flashdecoding}, predictions are computed in parallel with ongoing token generation, ensuring smoother and faster inference. The technique can be expressed as follows: at time step $t$, instead of waiting for the prediction of token $t-1$ to complete, the model computes the query $Q_t$ and performs the attention mechanism concurrently:

\begin{align}
    \hat{X}_t = \text{softmax}\left(\frac{Q_t K_{1:t}^\top}{\sqrt{d_k}}\right) V_{1:t}.
\end{align}

Here, $\hat{X}_t$ represents the output at time step $t$, while $K_{1:t}$ and $V_{1:t}$ are the cached keys and values from previous steps. By parallelizing this process, FlashDecoding++ reduces the token generation latency by decoupling computations from sequential dependencies.

\subsubsection{Model Parallelism and Pipeline Execution}
Model parallelism is a key strategy for scaling large models across multiple devices, particularly in large-scale LLMs where the model parameters are distributed over several GPUs. In frameworks like \textit{Megatron-LM} \citep{shoeybi2019megatron} and \textit{FlexGen} \citep{shen2023flexgen}, the model is split across GPUs, allowing each GPU to compute different parts of the model in parallel. The overall computation of a layer for a distributed model can be represented as:

\begin{align}
    \text{Forward Pass:} \quad X_{\text{output}} = f_{\text{GPU}_i}(X_{\text{input}}),
\end{align}

where $f_{\text{GPU}_i}$ denotes the function computed by GPU $i$, processing its portion of the model in parallel with other GPUs. Similarly, pipeline parallelism distributes different layers of the model across multiple devices. If the model is divided into $L$ layers across $N$ devices, each device handles a subset of the layers $\{L_1, L_2, \dots, L_N\}$, enabling the concurrent execution of different parts of the model.

\subsubsection{Mixed Precision and Low-Bit Inference}
Mixed precision inference is commonly used to reduce both memory and computational demands by executing non-critical operations in lower precision, such as FP16 or BF16, while maintaining full precision (FP32) for crucial operations \citep{micikevicius2018mixed}. The overall computational savings can be written as:

\begin{align}
    C_{\text{mixed}} = \sum_{i=1}^{n_{\text{ops}}} C_i \cdot p_i,
\end{align}

where $C_i$ represents the computational cost of operation $i$, and $p_i$ is the precision factor (1 for FP32, 0.5 for FP16). 

Extending this, \textit{Fast and Efficient 2-bit LLM Inference} \citep{zhou2023efficient} introduces low-bit inference by using 2/4/16-bit weight matrices. The quantized weights $W_q$ are dequantized asynchronously during inference:

\begin{align}
    W_q = \frac{W - W_{\min}}{W_{\max} - W_{\min}} \cdot (2^b - 1),
\end{align}

where $W$ represents the original weight matrix, $W_{\min}$ and $W_{\max}$ are the minimum and maximum values of $W$, and $b$ is the number of bits (e.g., 2, 4, or 16). This reduces memory bandwidth requirements while maintaining accuracy through asynchronous dequantization, ensuring efficient LLM inference.



% \subsection{Systematic Design in Model Compression}
% While quantization, knowledge distillation, and pruning all provide model-level optimization for reducing computational resources, there is currently a trend toward systematic design in model compression. System design of LLMs is a branch of computer system architecture that focuses on the storage implementation of basic memory elements, such as bytes. All electronic devices' memory storage is represented by units like GB or TB, and all files must be decoded to fit into a sequential byte format for storage.

% \subsubsection{Data Storage and Management}
% In computer systems, KV cache is a widely used technique for acceleration, storing key-value pairs such as student ID (key) and their basic information (value) in a sequential cache for acceleration. However, traditional sequential storage methods have drawbacks in LLM applications. According to \citet{kwon2023}, for the deployment of a 13B LLM on an NVIDIA V100 GPU, KV cache will consume more than 30\% of GPU storage, but these computational resources are greatly wasted due to reserved, internal fragmentation, and external fragmentation. To solve this problem, the authors developed PagedAttention, which allows continuous KV cache to be stored in non-contiguous memory space. PagedAttention introduces block table translation into storage, storing LLM requests as continuous space in "virtual memory." After block table translation, these requests are translated into pre-computed non-contiguous space in LLMs for memory efficiency. PagedAttention functions like a "docker scheduler" for memory, placing KV-cache "containers" in available spaces rather than in sequential order. Empirical results show that PagedAttention can save up to 9.79\% of memory usage through parallel sampling and up to 55.16\% through beam search, proving its efficiency in reducing computational resources.

% \subsubsection{Cache Eviction}
% In addition to PagedAttention, another notable work in model compression system design is StreamingLLM \citep{xiao2024}. Traditional KV storage methods such as dense attention and window attention lead to excessive memory usage and increasing latency in the decoding stage, degrading model performance as the sequence grows. To address this, \citet{xiao2024} developed an advanced cache eviction method called StreamingLLM. They revealed a phenomenon of "attention sink," where initial k-v tokens significantly impact language modeling tasks. Based on this finding, StreamingLLM stabilizes the attention sink tokens during computation while rolling the KV cache to retrieve the most recent tokens. As a result, it greatly reduces computational memory usage for LLMs from a magnitude level (O(TL\(^2\)) → O(TL)) and accelerates inference by 22.2x per token, proving its efficiency in reducing computational resources and even accelerating inference speed.

% \subsubsection{Computer Network Optimization}

% Some design such as \cite{liu2024cachegenkvcachecompression} optimize the cache usage in network transmission of prompt and KV cache.

% \subsection{Hardware Model Compression}

% The use of domain-specific hardware accelerators has been used as the most viable solution to the model compression on general-purpose hardware. \cite{9043731}\cite{9534870}

% \subsubsection{FGPA}
% \subsubsection{GPU}
% \subsubsection{in-memory\\flash}

==> contents/visllm_system.tex <==
% \section{System Design for Visual LLMs}

% Efficient system design for Visual Large Language Models (VLLMs) is crucial for overcoming computational and memory challenges caused by the large number of visual tokens and the complex attention mechanisms involved. This section presents a comprehensive overview of optimization strategies categorized into Token Reduction, Sparsity-Aware Optimization, and Key-Value (KV) Cache Compression. Detailed frameworks, equations, and examples of state-of-the-art methods are provided to illustrate these strategies.

% \subsection{Token Reduction Strategies}

% Visual tokens encode spatial information but often contain redundancy, particularly in deeper layers of VLLMs. Token reduction techniques aim to eliminate this redundancy while maintaining model performance.

% Token reduction can be formalized as a constrained optimization problem:
% \begin{align}
%     \min_{M, \hat{X}} \|X - (\hat{X} \odot M)\|^2 + \lambda \cdot \text{FLOPs}(M),
% \end{align}
% where:
% \begin{itemize}
%     \item \(X\): Original token embeddings.
%     \item \(M \in \{0, 1\}^T\): Binary mask for token selection.
%     \item \(\hat{X}\): Reduced token representations.
%     \item \(\lambda\): Trade-off parameter controlling the balance between computational cost and accuracy.
% \end{itemize}

% \subsubsection{Token Reduction by Layer-Wise Pruning}
% PyramidDrop reduces token redundancy by pruning low-importance tokens at the end of each stage:
% \begin{align}
%     R_t = \frac{\sum_{i \in \text{Neighbors}(t)} \text{Sim}(X_t, X_i)}{\|\text{Neighbors}(t)\|},
% \end{align}
% where \(R_t\) represents the redundancy score of token \(t\), and \(\text{Sim}(\cdot)\) is a similarity metric, such as cosine similarity. After computing redundancy scores, a fraction \(\alpha_l\) of the least significant tokens are pruned:
% \begin{align}
%     T_l = T_0 \cdot (1 - \alpha_l),
% \end{align}
% where \(T_l\) denotes the token count at layer \(l\). PyramidDrop achieves a 40\% reduction in training time and 55\% FLOPs savings while maintaining task performance \citep{pyramiddrop}.

% \subsubsection{Token Reduction by Compact Token Summarization}
% Victor introduces a register mechanism that aggregates visual tokens into compact representations:
% \begin{align}
%     X_{\text{register}}^{(k)} = \text{Aggregate}(X_{\text{visual}}^{(k-1)}),
% \end{align}
% where \(\text{Aggregate}\) pools visual token information into registers. Subsequent layers operate only on the summarized \(X_{\text{register}}\), reducing computational complexity:
% \begin{align}
%     \mathcal{O}((Q + R) \cdot N_{\text{params}}),
% \end{align}
% where \(Q\) is the number of text tokens, \(R\) is the number of register tokens, and \(R \ll T_0\). Victor improves inference throughput by 3.3$\times$ with less than a 4\% performance drop \citep{victor}.

% \subsection{Sparsity-Aware Optimization}

% Attention scores in VLLMs exhibit sparsity, offering opportunities to focus computation on significant tokens and ignore less relevant ones.

% ZipVL dynamically adjusts token retention ratios across layers based on the distribution of attention scores:
% \begin{align}
%     \rho_l = g(\bar{A}_l),
% \end{align}
% where \(\bar{A}_l\) is the mean attention score of tokens in layer \(l\), and \(g(\cdot)\) maps attention scores to retention ratios. Tokens are retained based on a saliency threshold:
% \begin{align}
%     X_{\text{retained}} = \{X_t \mid S_t > \tau\},
% \end{align}
% where \(S_t\) is the saliency score, and \(\tau\) is a dynamic threshold. ZipVL accelerates the prefill phase by 2.6$\times$ and reduces memory usage by 50\%, with a negligible accuracy loss of 0.2\% \citep{zipvl}.

% \subsection{Key-Value (KV) Cache Compression}

% The KV cache stores intermediate results during autoregressive decoding, creating a significant memory bottleneck for VLLMs due to the high number of tokens.

% VL-Cache compresses the KV cache by adapting precision levels based on token saliency:
% \begin{align}
%     \text{KV}_{\text{compressed}} = 
%     \begin{cases} 
%         \text{High-Precision}(X_t) & S_t > \tau, \\
%         \text{Low-Precision}(X_t) & S_t \leq \tau,
%     \end{cases}
% \end{align}
% where \(S_t\) is the saliency score of token \(t\), and \(\tau\) is the threshold for saliency. VL-Cache reduces memory usage by up to 90\% and improves decoding latency by 7$\times$ \citep{vlcache}.

% \subsection{Unified Optimization Objective}
% The strategies discussed can be combined into a unified optimization framework:
% \begin{align}
%     \min_{M_l, \hat{X}_l} \sum_{l=1}^{N_L} \|X_l - (\hat{X}_l \odot M_l)\|^2 + \lambda \cdot \text{Cost}(M),
% \end{align}
% where \(M_l\) represents binary masks for each layer \(l\), and \(\text{Cost}(M)\) reflects computational or memory overhead.

% \subsection{Applications in LLMs}
% Token reduction methods are widely applicable in both NLP-based LLMs and visual transformers. In LLMs, pruning and merging can be used to reduce the number of word tokens processed, thus improving inference speed with minimal impact on language understanding tasks \citep{goyal2020powerbert, kim2021learned, wan2023text} or domain-specific CILP-style pre-training~\citep{wan2024med, liu2024zero, liu2024etp}. In ViTs, token merging is particularly useful in image and video processing tasks, where spatial redundancy in adjacent tokens (representing image patches) can be leveraged to increase efficiency \citep{bolya2023tome}.

% Empirical results have shown that token merging can achieve significant speedups. For instance, in ViTs, ToMe can double throughput with minimal accuracy degradation, reducing the number of tokens by up to 98\% while maintaining performance on benchmarks like ImageNet \citep{bolya2023tome}. Similarly, token pruning has been shown to be effective in LLMs, where magnitude-based methods like Power-BERT \citep{goyal2020powerbert} reduce token count without re-training.

\subsection{System Design for Visual LLMs}

Designing systems for Visual Large Language Models (VLLMs) requires addressing significant computational and memory bottlenecks caused by high-dimensional visual tokens and complex attention mechanisms. This section discusses four optimization strategies: Token Reduction, Sparsity-Aware Optimization, Key-Value (KV) Cache Compression, and Unified Multi-Objective Frameworks, each supported by theoretical formulations and references to state-of-the-art methods.

\subsubsection{Token Reduction Strategies}

Visual tokens encode rich spatial and semantic information but often contain redundancy, particularly in deeper layers of VLLMs. Token reduction techniques aim to identify and eliminate this redundancy while retaining the necessary representational power. Let \( X \in \mathbb{R}^{T \times d} \) represent the token embeddings at a given layer, where \( T \) is the token count and \( d \) is the embedding dimension. The problem of token reduction can be formalized as minimizing reconstruction error under computational constraints:
\[
\min_{M, \hat{X}} \|X - (\hat{X} \odot M)\|_F^2 + \lambda \cdot \mathcal{C}(M) + \mu \cdot \mathcal{R}(M, \hat{X}),
\]
where \( M \in \{0, 1\}^T \) is a binary mask indicating token retention, \( \hat{X} \) is the reduced representation, \( \mathcal{C}(M) \) represents computational cost, and \( \mathcal{R}(M, \hat{X}) \) enforces regularization constraints such as spatial consistency. PyramidDrop adopts this framework by computing redundancy scores for each token based on local similarity metrics \citep{pyramiddrop}. Similarly, Victor leverages token summarization mechanisms, where token embeddings are aggregated into compact registers to reduce computation by over 3$\times$ with minimal accuracy loss \citep{victor}.

\subsubsection{Sparsity-Aware Optimization}

Attention mechanisms in VLLMs naturally exhibit sparsity, where a small subset of tokens often dominates attention computations. Exploiting this sparsity reduces computational costs by focusing only on high-saliency tokens. Let \( A \in \mathbb{R}^{T \times T} \) represent the attention matrix at a given layer, where \( A_{ij} \) denotes the attention weight between tokens \( i \) and \( j \). Sparsity-aware optimization selects a subset of tokens \( S = \{t \mid S_t > \tau\} \), where \( S_t = \sum_{j=1}^T A_{tj} \) represents the token's saliency score and \( \tau \) is a dynamically determined threshold. The optimization problem can be expressed as:
\[
\max_{\rho_l} \sum_{l=1}^{N_L} \rho_l \cdot \sum_{t \in S} \log\Big(1 + \frac{S_t}{\tau}\Big) - \kappa \cdot \mathcal{C}(\rho_l),
\]
where \( \rho_l \) denotes the retention ratio at layer \( l \), \( \mathcal{C}(\rho_l) \) is the computational cost associated with retaining tokens, and \( \kappa \) balances performance and cost. Methods like ZipVL dynamically adjust \( \rho_l \) across layers based on the attention distribution \citep{zipvl}, achieving over 50\% memory savings with minimal accuracy degradation.

\subsubsection{Key-Value (KV) Cache Compression}

Autoregressive decoding in VLLMs requires maintaining a Key-Value (KV) cache, which stores intermediate outputs for all tokens, creating significant memory overhead. Adaptive KV cache compression addresses this by adjusting the precision of stored tokens based on their importance. Let \( K, V \in \mathbb{R}^{T \times d} \) represent the key and value matrices. The optimization for adaptive precision is:
\[
\min_{\hat{K}, \hat{V}} \|K - \hat{K}\|_F^2 + \|V - \hat{V}\|_F^2 + \gamma \cdot \sum_{t=1}^T P_t \cdot \mathcal{C}(P_t),
\]
where \( \hat{K} \) and \( \hat{V} \) are the compressed representations, \( P_t \) denotes the precision level for token \( t \), and \( \mathcal{C}(P_t) \) quantifies the cost of using a specific precision. Precision levels can be dynamically assigned as \( P_t = \text{argmax}_{p \in \{\text{FP32}, \text{FP16}, \text{INT8}\}} \Big\{S_t \cdot \text{Utility}(p)\Big\} \), where \( S_t \) is the token saliency score and \( \text{Utility}(p) \) reflects the precision's effectiveness. VL-Cache achieves up to 90\% memory reduction with a 7$\times$ improvement in decoding latency \citep{vlcache}.

\subsubsection{Unified Optimization Framework}

The discussed strategies can be integrated into a unified multi-objective optimization framework to balance accuracy, computational efficiency, and memory usage. Let \( \mathcal{L}_{\text{task}} \) denote the primary task loss (e.g., classification or generation), and \( \mathcal{C} \) represent the overall cost function. The unified optimization objective is:
\[
\min_{\{M_l, \hat{X}_l, \rho_l, P_t\}} \mathcal{L}_{\text{task}} + \lambda \cdot \sum_{l=1}^{N_L} \|X_l - (\hat{X}_l \odot M_l)\|_F^2 + \mu \cdot \mathcal{R}(M_l, \hat{X}_l) + \kappa \cdot \mathcal{C}(M_l, \rho_l, P_t),
\]
where \( M_l \) is the binary mask for layer \( l \), \( \rho_l \) is the sparsity ratio, \( P_t \) denotes the precision level, and \( \mathcal{R}(M_l, \hat{X}_l) \) enforces structural regularization. The cost function \( \mathcal{C}(M_l, \rho_l, P_t) \) incorporates memory, latency, and computational constraints, ensuring that the model remains efficient across various tasks. This unified framework has been successfully applied in PyramidDrop, ZipVL, and VL-Cache, showcasing its adaptability across domains \citep{pyramiddrop, victor, zipvl, vlcache}.


==> figures/KVcache.tex <==
\begin{tikzpicture}[node distance=2cm]

% Styles
\tikzstyle{startstop} = [rectangle, rounded corners, minimum width=3cm, minimum height=1cm,text centered, draw=black, fill=red!30]
\tikzstyle{process} = [rectangle, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=blue!30]
\tikzstyle{arrow} = [thick,->,>=stealth]

% % Nodes
% \node (start) [startstop] {Input Prompt};
% \node (query) [process, below of=start] {Generate Query (Q)};
% \node (cachecheck) [process, below of=query] {Check KV Cache};
% \node (updatecache) [process, right of=cachecheck, xshift=5cm] {Update KV Cache \\ $\mathbf{K}_{\text{low}} = \mathbf{U} \mathbf{K}, \, \mathbf{V}_{\text{low}} = \mathbf{V} \mathbf{V}^\top$};
% \node (attention) [process, below of=cachecheck, yshift=-1.5cm] {Compute Attention \\ $\hat{\mathbf{X}}_t = \text{softmax} \left( \frac{\mathbf{Q}_t \mathbf{K}_{1:t}^\top}{\sqrt{d_k}} + \mathbf{B}_t \right) \mathbf{V}_{1:t}$};
% \node (output) [startstop, below of=attention] {Generate Output Token};
% \node (opt) [process, below of=updatecache, yshift=-3cm, xshift=-3cm] {Optimize KV Cache \\ $\min_{\mathbf{K}_{\text{low}}, \mathbf{V}_{\text{low}}} \| \mathbf{K} - \mathbf{K}_{\text{low}} \|_F^2 + \| \mathbf{V} - \mathbf{V}_{\text{low}} \|_F^2 + \lambda \mathcal{C}(\mathbf{K}_{\text{low}}, \mathbf{V}_{\text{low}})$};

% % Arrows
% \draw [arrow] (start) -- (query);
% \draw [arrow] (query) -- (cachecheck);
% \draw [arrow] (cachecheck) -- (attention);
% \draw [arrow] (cachecheck.east) -- ++(1,0) |- (updatecache.west);
% \draw [arrow] (updatecache) -- ++(0,-1.5) |- (attention.east);
% \draw [arrow] (attention) -- (output);
% \draw [arrow] (updatecache.south) -- ++(0,-1.5) -| (opt.north);

% Nodes
\node (start) [startstop] {Input Prompt};
\node (query) [process, below of=start] {Generate Query (Q)};
\node (cachecheck) [process, below of=query] {Check KV Cache};
\node (updatecache) [process, right of=cachecheck, xshift=5cm] {Update KV Cache \\ $\mathbf{K}_{\text{low}} = \mathbf{U} \mathbf{K}, \, \mathbf{V}_{\text{low}} = \mathbf{V} \mathbf{V}^\top$};
\node (attention) [process, below of=cachecheck, yshift=-1.5cm] {Compute Attention \\ $\hat{\mathbf{X}}_t = \text{softmax} \left( \frac{\mathbf{Q}_t \mathbf{K}_{1:t}^\top}{\sqrt{d_k}} + \mathbf{B}_t \right) \mathbf{V}_{1:t}$};
\node (output) [startstop, below of=attention, yshift=-1cm] {Generate Output Token}; % 下移输出块
\node (opt) [process, below of=updatecache, yshift=-2cm] {Optimize KV Cache \\ $\min_{\mathbf{K}_{\text{low}}, \mathbf{V}_{\text{low}}} \| \mathbf{K} - \mathbf{K}_{\text{low}} \|_F^2 + \| \mathbf{V} - \mathbf{V}_{\text{low}} \|_F^2 + \lambda \mathcal{C}(\mathbf{K}_{\text{low}}, \mathbf{V}_{\text{low}})$};

% Arrows
\draw [arrow] (start) -- (query);
\draw [arrow] (query) -- (cachecheck);
\draw [arrow] (cachecheck) -- (attention);
\draw [arrow] (cachecheck.east) -- ++(1,0) -- (updatecache.west); % 使用直线连接
\draw [arrow] (updatecache) -- (opt); % 直线连接
\draw [arrow] (attention) -- (output);
\draw [arrow] (updatecache.east) -- ++(1,0) -- ++(0,-1.5) -- ++(-6.5,0) -- (attention.east);

\end{tikzpicture}


==> figures/KVcache_sys.tex <==
% Adjusted Visualization Framework for Text LLM
\begin{tikzpicture}[node distance=1.5cm and 2.5cm]

% Main components
\node (kvdesign) [main] {KV Cache Design};
\node (tokenred) [main, right=of kvdesign] {Token Reduction};
\node (optimization) [main, right=of tokenred] {Optimization Techniques};

% KV Cache Submodules
\node (framework) [sub, below=of kvdesign, yshift=-0.5cm] {Mathematical Framework};
\node (advanced) [sub, below=of framework] {Advanced Formulations};
\node (optimizationkv) [sub, below=of advanced] {Inference Optimizations};

% Token Reduction Submodules
\node (pruning) [sub, below=of tokenred, yshift=-0.5cm] {Token Pruning};
\node (merging) [sub, below=of pruning] {Token Merging};

% Optimization Submodules
\node (dynamic) [sub, below=of optimization, yshift=-0.5cm] {Dynamic Allocation};
\node (sparsity) [sub, below=of dynamic] {Sparsity Awareness};
\node (precision) [sub, below=of sparsity] {Precision Scaling};
\node (execution) [sub, below=of precision] {Distributed Execution};

% Impact Analysis (Shifted to balance layout)
\node (impact) [secondary, below left=of optimization, yshift=-0.5cm, xshift=1.5cm] {Impact Analysis};
\node (latency) [sub, below=of impact, yshift=-0.5cm] {Latency Reduction};
\node (memory) [sub, below=of latency] {Memory Efficiency};
\node (scalability) [sub, below=of memory] {Scalability};

% Connections for KV Cache
\draw [arrow] (kvdesign) -- (framework);
\draw [arrow] (framework) -- (advanced);
\draw [arrow] (advanced) -- (optimizationkv);

% Connections for Token Reduction
\draw [arrow] (tokenred) -- (pruning);
\draw [arrow] (pruning) -- (merging);

% Connections for Optimization
\draw [arrow] (optimization) -- (dynamic);
\draw [arrow] (dynamic) -- (sparsity);
\draw [arrow] (sparsity) -- (precision);
\draw [arrow] (precision) -- (execution);

% Connections for Impact Analysis
\draw [arrow] (impact) -- (latency);
\draw [arrow] (latency) -- (memory);
\draw [arrow] (memory) -- (scalability);

% Cross-module relationships
\draw [arrow] (kvdesign.east) to[out=0, in=180] (tokenred.west);
\draw [arrow] (optimization.south) to[out=-90, in=90] (impact.north);
\draw [arrow] (tokenred.south) to[out=-90, in=180] (pruning.west);

\end{tikzpicture}


==> figures/taxonomy.tex <==
% \definecolor{hidden-draw}{rgb}{0.5, 0.5, 0.5}
% \definecolor{quant-color}{rgb}{0.0, 0.5, 0.0}  % Green for Quantization and Distillation
% \definecolor{sys-design-color}{rgb}{0.8, 0.0, 0.0}  % Red for Model-System Co-design

\definecolor{hidden-draw}{rgb}{0.5, 0.5, 0.5}
\definecolor{quant-color}{rgb}{0.0, 0.5, 0.0}  % Green for Quantization and Distillation
\definecolor{sys-design-color}{rgb}{0.8, 0.0, 0.0}  % Red for System Design
\definecolor{co-design-color}{rgb}{0.0, 0.0, 0.8}  % Blue for Model-System Co-design


\usetikzlibrary{trees}

% Define the leaf style
\tikzset{leaf/.style={draw, fill=quant-color!20}}

\begin{figure*}[!th]
    \resizebox{\textwidth}{!}{
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=left,
                font=\large,
                rectangle,
                draw=hidden-draw,
                rounded corners,
                align=left,
                minimum width=4em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                line width=0.8pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
                where level=1{fill=quant-color!30, font=\normalsize,}{},
                where level=2{fill=hidden-color!30, font=\normalsize,}{},
                where level=3{fill=sys-design-color!30, font=\normalsize,}{},
                where level=4{fill=co-design-color!30, font=\normalsize,}{},

                % ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
                % where level=1{fill=hidden-draw!20, font=\normalsize,}{},
                % match={Model Design}{fill=quant-color!30},
                % match={System Design}{fill=sys-design-color!30},
                % match={Model-System Co-design}{fill=co-design-color!30},
                % match={Quantization}{fill=quant-color!20},
                % match={Distillation}{fill=quant-color!20},
                % match={Pruning}{fill=quant-color!20},
                % match={KV Cache Compression}{fill=sys-design-color!20},
                % match={Parallelism}{fill=sys-design-color!20},
                % match={Memory Management}{fill=sys-design-color!20},
                % % match={Low-Level Optimization for GPUs}{fill=sys-design-color!20},
                % match={Mixture of Experts}{fill=co-design-color!20},
                % match={Mixed Precision Training}{fill=co-design-color!20},
            },
            [
                Efficient \\ Foundation \\ Models,
                [
                    Model Design, 
                    [
                        Quantization, 
                        [
                            Bitwise-Based
                            [
                                1-bit/2-bit \cite{su2025rotatekv, su2025akvq, zheng2024bidm}
                            ]
                            [
                                4-bit \cite{chmiel2023accurate, liu2023llm, ashkboos2024quarot, lee2025qrazor}
                            ]
                            [
                                8-bit \cite{bhandare2019efficient, jin2022f8net, zhao2023atom}
                            ]
                        ]
                        [
                            Method-Based
                            [
                                PTQ (Post-Training Quantization) \cite{E-li2024efficient,jacob2018quantization}, leaf
                            ]
                            [
                                QAT (Quantization-Aware Training) \cite{nagel2021white,esser2019learned}, leaf
                            ]
                        ]
                    ]
                    [
                        Distillation, 
                        [
                            Soft Knowledge Distillation, 
                            [
                                Classical KD \cite{hinton2015distilling}, leaf
                            ]
                            [
                                Temperature-Scaled KD \cite{li2022asymmetric}, leaf
                            ]
                        ]
                        [
                            Hard Knowledge Distillation, 
                            [
                                Hard Label KD \cite{hou2020dynabert}, leaf
                            ]
                            [
                                Program-Aided Distillation (PaD) \cite{shridhar2022distilling}, leaf
                            ]
                        ]
                    ]
                    [
                        Pruning, 
                        [
                            Unstructured Pruning \cite{frankle2018lottery,gale2019state}, leaf
                        ]
                        [
                            Structured Pruning \cite{wang2024loma,li2022deja}, leaf
                        ]
                    ]
                ]
                [
                    System Design, 
                    [
                        KV Cache Compression \cite{peng2022cachegen,huang2023cachegen,kwon2023efficient}, leaf
                    ]
                    [
                        Parallelism \cite{shoeybi2019megatron,xu2021colossal}, leaf
                    ]
                    [
                        Contextual Sparsity \cite{li2022deja,kurtz2020inducing,quest}, leaf
                    ]
                    [
                        Memory Management \cite{dao2022flashattention,kwon2023efficient,lee2024infinigen, alizadeh2023llm}, leaf
                    ]
                    [
                        Low-Level Optimization for GPUs \cite{weng2023transformer,girgis2021effective}, leaf
                    ]
                ]
                [
                    Model-System Co-design,
                    [
                        Mixture of Experts \cite{Collobert2001, Rasmussen2001, Eigen2014, Theis2015NeurIPS, Aljundi2017CVPR}, leaf
                    ]
                    [
                        Fine-tuning with System Optimizations \cite{hu2021lora,xu2023efficient, zhang2023lora, ding2023sparse, wang2024loma}, leaf
                    ]
                    [
                        Mixed Precision Training \cite{shen2023flexgen,micikevicius2018mixed,xu2022survey}, leaf
                    ]
                    [
                        Efficient Model Inference on Optimized Systems \cite{fastertransformer2021,tensorrt2022}, leaf
                    ]
                    [
                        Model Compression with FlexGen and System Optimizations \cite{shen2023flexgen, wang2024loma}, leaf
                    ]
                ]
            ]
        \end{forest}
    }
    \caption{Efficient Foundation Models Overview}
    \label{fig:llm_optimization_overview}
\end{figure*}


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/LLMs.tex <==
% \begin{table}[h]
% \centering
% \caption{Open Source Large Language Models (LLMs)}
% \begin{tabular}{|c|c|c|l|}
% \hline
% \textbf{Model}   & \textbf{Year} & \textbf{Parameters (B)} & \textbf{Source Link} \\ \hline
% LLaMa            & 2023          & 13                      & \url{https://github.com/facebookresearch/llama} \\ \hline
% GPT-3            & 2020          & 175                     & \url{https://openai.com/gpt-3} \\ \hline
% FlexGen          & 2023          & -                       & \url{https://github.com/FMInference/FlexGen} \\ \hline
% PaLM             & 2022          & 540                     & \url{https://github.com/google-research/palm} \\ \hline
% CacheGen         & 2023          & -                       & \url{https://github.com/cachegen-project} \\ \hline
% Deepseek         & 2023          & -                       &  \\ \hline
% Qwen         & 2023          & -                       &  \\ \hline
% GLM         & 2023          & -                       &  \\ \hline
% \end{tabular}
% \end{table}

\begin{table}[h]
\centering
\small % This shrinks the table text size
\caption{Open Source LLMs with Parameters}
\begin{tabular}{|c|c|c|c|l|}
\hline
\textbf{Model}   & \textbf{Year} & \textbf{Parameters (B)} & \textbf{Variants}  & \textbf{Source Link} \\ \hline
LLaMa            & 2023          & 7, 13, 30, 65           & LLaMA-1, LLaMA-2, LlaMA-3     & \url{https://github.com/facebookresearch/llama} \\ \hline
GPT-2            & 2020          & 175                     & Ada, Babbage, Curie, Davinci & \url{https://openai.com/gpt-3} \\ \hline
FlexGen          & 2023          & -                       & N/A                   & \url{https://github.com/FMInference/FlexGen} \\ \hline
PaLM             & 2022          & 8, 62, 540              & PaLM, PaLM 2          & \url{https://github.com/google-research/palm} \\ \hline
CacheGen         & 2023          & -                       & N/A                   & \url{https://github.com/cachegen-project} \\ \hline
Deepseek         & 2023          & 2, 7                    & V1, V2, V2.5           & \url{https://huggingface.co/deepseek-ai} \\ \hline
Qwen             & 2023          & 7, 14                   & V1, V2           & \url{https://qwenlm.github.io/} \\ \hline
GLM              & 2023          & 10, 130                 & GLM-130B, GLM-10B     & \url{https://github.com/THUDM/GLM} \\ \hline
OPT              & 2022          & 1.3, 2.7, 6.7, 30, 66   & OPT family            & \url{https://github.com/facebookresearch/opt} \\ \hline
Bloom            & 2022          & 176                     & Bloom, BloomZ         & \url{https://huggingface.co/bigscience/bloom} \\ \hline
MPT              & 2023          & 7, 30                   & MPT-7B, MPT-30B       & \url{https://www.mosaicml.com/mpt} \\ \hline
Falcon           & 2023          & 7, 40                   & Falcon-7B, Falcon-40B & \url{https://huggingface.co/tiiuae/falcon-7b} \\ \hline
Pythia           & 2022          & 1, 2.8, 6.9, 12, 19, 27 & Multiple              & \url{https://huggingface.co/EleutherAI/pythia} \\ \hline

\end{tabular}
\end{table}
